How do centrality measures choose the root of trees?

Centrality measures are widely used to assign importance to graph-structured data. Recently, understanding the principles of such measures has attracted a lot of attention. Given that measures are diverse, this research has usually focused on classes of centrality measures. In this work, we provide a different approach by focusing on classes of graphs instead of classes of measures to understand the underlying principles among various measures. More precisely, we study the class of trees. We observe that even in \fix{the} case of trees, there is no consensus on which node should be selected as the most central. To analyze the behavior of centrality measures on trees, we introduce a property of \emph{tree rooting} that states a measure selects one or two adjacent nodes as the most important, and the importance decreases from them in all directions. This property is satisfied by closeness centrality but violated by PageRank. We show that, for several centrality measures that root trees, the comparison of adjacent nodes can be inferred by \emph{potential functions} that assess the quality of trees. We use these functions to give fundamental insights on rooting and derive a characterization explaining why some measure root trees. Moreover, we provide an almost liner-time algorithm to compute the root of a graph by using potential functions. Finally, using a family of potential functions, we show that many ways of tree rooting exist with desirable properties.

==> PODScomments.tex <==
\begin{itemize}
	
	\item $\checkmark$  I do not think that it is a good idea to have essentially no references in the introduction.
	
	\item $\checkmark$ p1: "To understand what distiguish" -> distinguishes
	
	\item $\checkmark$ p3: "what we could expect from a root" You should give a more compelling motivation here. I see no reason what central vertices should not be distributed in the tree.
	
	\item $\checkmark$ p5: The sentence starting with "Notice that the naive approach" is clearly wrong for the case in which the actual computation of the centrality measure for each individual pair takes nontrivial time.
	
	\item $\checkmark$ p5: "This step discard" -> discards
	
	\item $\checkmark$ p7: "The rooting-tree property implies the structure of centralities in every possible graph". I have no idea what this sentence is supposed to say. Also why should there be any relation to graphs that are not trees?
	
	\item $\checkmark$ p7: "admit potential function" -> admits
	
	\item $\checkmark$ p7: "imposes on the potential function" -> imposes
	
	\item $\checkmark$ p7: "every trees T" -> every tree
	
	\item $\checkmark$ p7: "The purpose of this family has two goals" This is just gibberish. What are you trying to say?
	
	\item $\checkmark$ p7: "set of hypothesis" -> hypotheses
	
	\item $\checkmark$ p7: "definition of monoids" Get rid of space before the comma.
	
	\item $\checkmark$ p8: "To makes them necessary" -> make; or even better change the formulation to "To get a necessary condition" or similar.
	
	\item $\checkmark$  p8: "the range of function" -> the function
	
	\item Maybe in the introduction it could be mentioned that some (and which) measures are defined in Section 2.
	
	\item $\checkmark$ "Even in the case of tree structures, centrality measures varies
	significantly."-> vary
	
	\item $\checkmark$ "there exists an isomorphism f ...  such that ... if, and only if, ...." Rather say bijection than isomorphism, because the second part defines the term isomorphism.
	
	\item $\checkmark$ "that given a pair (v,g) it assigns a score
	C(v,G) to v depending on its graph G" doesn't it simply assign a score to each pair (v,G)?
	
	\item $\checkmark$ "is a shortest paths" -> path
	
	\item $\checkmark$ "Note that since the distance between two vertices in different connected
	components is not defined, we have to define the sum of distances
	just inside a connected component." You can hardly give too many explanations, but this might be an exception. Besides, the distance between nodes in different components *is* defined: it is infinite.
	
	\item $\checkmark$
	"The intuition behind closeness centrality is simple: the closer
	a vertex is to everyone in the network the more important it is." But it is less clear that the actual definition indeed captures this intuition.
	
	\item $\mathord{?}$ Maybe it could be stressed even more, right at the beginning of Section 4, that potential functions are about subtrees
	
	\item $\checkmark$ It is not clear why the claimed equality for the size of A(u,T) should hold. At least, I failed to verify it for a path of length 5 with inner nodes u,v.
	
	\item $\mathord{?}$ I'd recommend to not call the property of Lemma 4.3 "symmetric". The definition has no symmetry involved and thus the name does not appeal to intuition. Something like "subtree-property" seems more appropriate to me (but please do not feel obliged…). That the notion coincides with symmetricity of C is a *result*.
	
	\item $\mathord{?}$ In the proof of 4.6 the variable v is overloaded.
	
	\item $\times$ Algorithm 1, line 3 should use the *size* of the neighbourhood
	
	\item $\mathord{?}$ In Algorithm1, it is not clear to me how the computation of the f-values of neighbours synchonizes with the advance of the algorithm. However, since at most two values per edge are needed, they can be computed in advance.
	
	\item $\checkmark$ Prop. 6.5: v in V(T) cap V(T') seems redundant since T' is a subtree of T
	
	\item $\checkmark$ I assume in the definition of monotonic over subtrees it should be ell-bar instead of f.
	
	\item $\times$ It is not clear why PageRank, EigenVector and a few others are mentioned in the text (in particular, on p 5) if the developed machinery is not applicable to them (would, for instance, PageRank be interesting on trees?). These centrality measures are not even defined in the text, so, it's difficult to assess the claims.
	
	\item $\checkmark$ The meaning of "runs almost linearly" becomes clear only half a page below - it looks like it's O(n log n), which is obviously not linear. Why do the authors use the misleading term then? One could understand it as O(n log log log n), for example.
	
	\item $\checkmark$ Proposition 5.1 is very difficult to understand due to the wide range of names for the same nodes - $w_1$ is u, and $w_n$ is v, and all components of both pairs are used together in the same formulas, which does not make it easy to get through. Why not "Let ...  and $w_1...w_n$ be the unique path connecting some $w_1, w_n \in V(T)$"? 
	
	\item $\times$ It is not very clear in the text immediately below the definition of C(v,T) in Example 6.4 that it begins an argument to show that C(v,T) is a centrality measure.
	
	\item $\times$ If ordered monoids are defined on p 8, it would be helpful to have the definition of the order on commutative monoids on p 7, for example.
	
	\item $\checkmark$ "centrality measures vary (not varies) significantly"
	
	\item $\checkmark$ There should be no - in "Rooting-tree" in Definition 3 (or, better, it should be called Tree Rooting). The same applies to the occurrences around Proposition 3.5. Only of p 5, the authors use "the rooting-tree property", which makes a bit more sense (unlike plain Rooting-Tree).
	
	\item $\mathord{?}$ Insert , before "if" in Definition 3.1.
	
	\item $\checkmark$ In Definition 3.6, "it holds" should be replaced by "it holds that", or better still, use "if $(u_1, T_{u_1},v) = (u_2, T_{u_2},v)$, then ... ". Same in Definition 6.1.
	
	\item $\checkmark$ "through the lens (not lenses) of potential functions"
	
	\item $\checkmark$ "satisfies "the" at-most-one-parent property"
	
	\item $\checkmark$ Insert , before "which" in the last line of the proof of Theorem 4.4.
	
	\item $\checkmark$ Remove "we get that" from Example 4.5.
	
	\item $\checkmark$ Proposition 4.6: There exists a centrality measure that root"s" trees but (remove it) does not admit a potential function.
	
	\item $\checkmark$ Remove the first "Then" from Proposition 5.1 (two thens in a single sentence is a bit too much).
	
	\item $\checkmark$ "the previous proposition" should be replaced by "Proposition 5.1"
	
	\item $\checkmark$ "to some extend" should be "to some extent".
	
	\item $\checkmark$ "developed in earlier sections" should be more specified - what are "earlier" sections?
	
	\item $\checkmark$ "The purpose of this family has two goals" does not make sense - is it "The purpose of this family is twofold"?
	
	\item $\checkmark$ "The previous theorem" should be "Theorem 7.4"
\end{itemize}

==> app-alternativeproof.tex <==
Definition 6 (a leaf attached to a graph has the higher centrality than its parent in the original graph) might seem undesirable. 
However, in the following theorem we show that it is necessary to obtain Theorem~\ref{Th:Theorem3}.
Specifically, if a centrality satisfies Isomorphism (isomorphic nodes in isomorphic graphs have the same centralities), Preserved order (Axiom 5) and Cut-vertex Increase (implied by Definition 5), then it satisfies property specified in Theorem~\ref{Th:Theorem3} if and only if it satisfies Leaf Beats Parent (implied by Definition 6).

\begin{theorem}\label{Th:Theorem3_simpler}
Let $C$ be a centrality measure that satisfies:
\begin{itemize}
\item \emph{Isomorphism}: if $\phi$ is an isomorphism between $G_1$ and $G_2$, then $C(v,G_1) = C(\phi(v), G_2)$ for every $v \in V(G_1)$. 
\item \emph{Preserved asymmetry} (Axiom 4)
\item \emph{Cut-vertex Increase}: for every two trees $T_1, T_2$ such that $V(T_1)\cup V(T_2) = \{v\}$ we get $C(v,T_1) \le C(v,T_1 \cup T_2)$.
\end{itemize}
Now, the following two properties are equivalent:
\begin{itemize}
\item[(i)] \emph{Leaf Beats Parent}: for every tree $T$ and node $v \not \in V(T)$, $C(u,T) < C(v, T + \{u,v\})$.
\item[(ii)] \emph{Theorem~\ref{Th:Theorem3}}: for every tree $T = (V,E)$ and node $v \in V(T)$ there exists at most one $u \in N(v)$ such that $C(u,T) \ge C(v,T)$.
\end{itemize}
\end{theorem}

\begin{proof}
(i) $\Rightarrow$ (ii): 
Fix an arbitrary tree $T$, node $v$ and let $u,w$ be two arbitrary neighbors of $v$ in tree $T$.
By removing edges $\{u,v\}$ and $\{v,w\}$ we get a decomposition of $T$ into 3 trees, $T_u, T_v, T_w$ containing $u,v,w$, respectively:
\[ T = T_v \cup T_u \cup T_w + \{u,v\} + \{v,w\}. \]
Without loss of generality assume $C(u,T_u) \ge C(w,T_w)$.
From Leaf Beats Parent we have $C(v, T_u + \{u,v\}) > C(u,T_u)$ and using Cut-vertex Increase we get $C(v, T_u \cup T_v + \{u,v\}) > C(u,T_u)$.
Based on our assumption also $C(v, T_u \cup T_v + \{u,v\}) > C(w,T_w)$.
This, combined with Preserved order, implies that $C(v,T) > C(w,T)$.
Hence, we just proved that out of every two neighbors at least one has smaller centrality than $v$ which implies the thesis.

(ii) $\Rightarrow$ (i):
Assume $C$ violates Leaf Beats Parent. 
We will show that it also violates Theorem 3.
Let $T$ be a tree and $u$ be a node such that $C(u,T) \ge C(v,T + \{u,v\})$.
Take a second tree $T'$ isomorphic to $T$ such that $u'$ corresponds to $u$.
From Isomorphism we know that $C(u',T') = C(u,T)$.
Let us construct a tree $T^*$ by adding $T'$ and edge $\{u',v\}$ to $T + \{u,v\}$: 
\[ T^* = T \cup T' + \{u,v\} + \{u',v\}. \]
From Preserved order we get:
\[ C(u',T^*) \ge C(v,T^*). \]
Analogously (or directly from Isomorphism) we get that $C(u,T^*) \ge C(v,T^*)$ which means Theorem 3 is not satisfied.
\end{proof}


==> app-axioms.tex <==
In this section, we introduce several axioms for rankings over trees, called tree centrality rankings, and we study their properties in the next sections. Recall that $\mathcal{V}$ is a fix enumerable set of vertices, and let $\cT$ be the set of all trees over finite subsets of $\mathcal{V}$. Let $\preceq$ be any centrality ranking over $\cT$.

\begin{axiom}[Closed under isomorphism] We say that $\preceq$ satisfies the \emph{closed under isomorphism} axiom if, and only if, for every pair of trees $T_1$ and $T_2$ such that there exists an isomorphism $h:V(T_1)\to V(T_2)$ then $(v,T_1) \equiv (h(v), T_2)$ for every vertex $v$ in $V(T_1)$.
\end{axiom}
In other words, thia axiom says that equivalence relation $\cong$ is a refinement of~$\equiv$. 

\begin{axiom}[Isolated vertex] We say that $\preceq$ satisfies the \emph{isolated vertex} axiom if, and only if, for every tree $T$ and $v \in V(T)$ it holds that $(v, T_v) \preceq (v, T)$ where $T_v = (\{v\}, \emptyset)$ is the trivial tree. Furthermore, $(v, T_v) \equiv (v, T)$ if, and only if, $T_v = T$. 
\end{axiom}

The previous axiom states that the trivial tree is a minimum element for the centrality ranking. Combined with the closed under isomorphism axioms, it implies that the trivial tree is the minimum of the ranking up to isomorphism.

\begin{axiom}[Weak monotonicity]
	We say that $\preceq$ satisfies \emph{weak monotonicity} axiom if, and only if, for every  tree $T$ and $v \in V(T)$ it holds that $(v, T) \preceq (v, T \cup T')$ for every tree $T'$ with $V(T)\cap V(T') = \{v\}$. Moreover,  $(v,T) \equiv (v, T \cup T')$ if, and only if, $T'$ is the trivial tree  $(\{v\},\emptyset)$.
\end{axiom}

\begin{axiom}[Strong monotonicity]
	We say that $\preceq$ satisfies \emph{strong monotonicity} axiom if, and only if, for every pair of trees $T_1, T_2$, and $v \in V(T_1) \cap V(T_2)$, if $(v, T_1) \preceq (v, T_2)$, then $(v, T_1 \cup T_3) \preceq (v, T_2\cup T_3)$ for every tree $T_3$ with $V(T_1)\cap V(T_3) = V(T_2) \cap V(T_3) = \{v\}$. 
\end{axiom}

\begin{axiom}[Rank monotonicity] We say that $\preceq$ satisfies \emph{rank monotonicity} axiom if, and only if, for every pair of disjoint trees $T_1$ and $T_2$ and for every $v_1 \in V(T_1)$ and $v_2 \in V(T_2)$, we have that $(v_1,T_1) \preceq (v_2,T_2)$ if, and only if,  $(v_1, (T_1 \cup T_2) + \{v_1,v_2\}) \preceq (v_2, (T_1\cup T_2) + \{v_1,v_2\})$.
\end{axiom}

The previous axioms talks about the monotonicity of the ranking when adding a tree or an edge. The next axioms talks about the rankings and the leafs of a tree.

\begin{axiom}[Leaf-beats-parent]
	 We say that $\preceq$ satisfies \emph{leaf-beats-parent} axiom if, and only if, for every tree $T$ and $v \in V(T)$it holds that $(v, T) \prec (u, T + \{v,u\})$ for every $u \notin V(T)$.
\end{axiom}

\begin{axiom}[Leaf monotonicity]
	We say that $\preceq$ satisfies \emph{leaf monotonicity} axiom if, and only if,  for every pair of trees $T_1$ and $T_2$, vertices $v_1 \in V(T_1)$ and $v_2 \in V(T_2)$, it holds that, if $(v_1, T_1) \preceq (v_2, T_2)$ then $(w, T_1 \cup\{w, v_1\}) \preceq (w, T_2 \cup\{w, v_2\})$ for every fresh vertex $w \not\in V(T_1)\cup V(T_2)$
\end{axiom}

The following axiom is a generalization of the previous axioms, and it is here for further studies. 

\begin{axiom}[Broken symmetry]
	We say that $\preceq$ satisfies \emph{broken symmetry} axiom if the following property holds. Let $T$ be a tree and $v_1\not=v_2$ vertices in $T$ such that $(v_1, T )\cong (v_2, T)$. For every $(v_1, T_1)$ and $(v_2, T_2)$ with disjoints trees $T_1$ and $T_2$ then $(v_1, T_1) \preceq (v_2, T_2)$ if, and only if, $(v_1, T \cup T_1\cup T_2)\preceq (v_2, T\cup T_1\cup T_2)$.
\end{axiom}



\subsubsection{Axioms relations and properties}

Even though the axioms defined previously are really simple and intuitive, they are not independent. In other word, given certain restrictions, some of the axioms became equivalent.

\begin{lemma}
	If a ranking $\preceq$ enjoys broken symmetry and close under isomorphism, then $\preceq$ enjoys rank monotonicity and strong monotonicity.
\end{lemma}
\begin{proof}
First, suppose we have $(v_1, T_1)$ and $(v_2, T_2)$. Define $T = (\{v_1,v_2\},\{v_1,v_2\})$ the edge tree containing $v_1$ and $v_2$. By broken symmetry we know that $(v_1, T_1)\preceq (v_2, T_2)$ if and only if $(v_1, T_1 \cup T_2 \cup T)\preceq(v_2, T_1 \cup T_2 \cup T)$ since $(v_1, T)\cong (v_2, T)$. This is exactly rank monotonicity statement.

In second place, for a fixed $T_3$ and $v$ in $T_3$ define the tree $T_3'\cong T_3$ such that $V(T_3)\cap V(T_3') = \emptyset$ and node $v'$ in $V(T_3')$ such that $(v, T_3)\cong (v', T_3')$. Therefore, for $T= T_3 \cup T_3' \cup \{v, v'\}$ then $(v, T)\cong(v', T)$. Now, for $T_1$ and $T_2$ such that $v\in V(T_1)$ and $v'\in V(T_2)$, if $(v, T_1)\prec (v', T_2)$ then, by broken symmetry, we have that $(v, T\cup T_1)\prec (v', T\cup T_2)$. Which implies that $(v, T_3\cup T_1)\preceq (v, T_3\cup T_2)$ by rank monotonicity and CUI.

\end{proof}



==> app-centrality-sets.tex <==
In this section we extend SG-centrality from vertices to set of vertices. For this, it is helpful to work with multigraphs, namely, undirected graphs with multi-edges. Formally, a multigraph $G$ is a triple $G = (V,E,r)$ such that $V$ is a finite non-empty set, $E$ is a finite set and $r: E \rightarrow \{\{v,v'\} \subseteq V \mid v \neq v'\}$. Intuitively, $E$ is a set of identifiers for edges and $r$ assigns identifiers to edges (i.e. pair of vertices). Note that there could be two different identifiers $e, e' \in E$ with $r(e) = r(e') = \{v, v'\}$, stating that there are two edges connecting $v$ with $v'$. 
We say that $G' = (V', E', r')$ is a submultigraph (or just subgraph for short) of $G$ if $V' \subseteq V$, $E \subseteq E'$, and $r' \subseteq r$. Similar than for normal graphs, we denote by $\sgu_G$ the set of all subgraphs of $G$. The notions of path, connected graph and strongly connected component is defined similar than before. 

It is straightforward to extend the notion of SG-centrality from graphs with single edges to graph with multi-edges. Here, we extend the notion of SG-centrality to set of vertices over graphs with multi-edges.
\begin{definition}
	Let $G = (V, E, r)$ be a multigraph. The Subgraph Centrality of a non-empty set $A \subseteq V$ in $G$ is defined as:
	$$
	\scen_{G}(A) \ = \ \log |\{G' \in \sgu_G \ \mid \ \forall \, (V', E', r') \in \scc(G'). \ V' \cap A \neq \emptyset\}|
	$$ 
\end{definition}
Intuitively, the extension to set of vertices is counting the amount of minimal subgraphs $G'$ of $G$ such that each strongly connected component of $G'$ contains at least one vertex of $A$. This definition is a generalization of the SG-centrality: if $A = \{v\}$ for some $v \in V$, then the subgraph $G'$ must be connected (i.e. exactly one strongly connected component) and must contain $v$. 

A good property of the SG-centrality for sets of vertices is that it can be reduced to computing the centrality of a single vertex in a multigraph (this is the main reason to consider multigraphs in this section).
For this, we need to introduce some notation. Let $A$ be a subset of vertices from a graph $G$. We define the graph $\collapse{G}{A}$ as the result of merging the nodes in $A$ to one node and keeping multi-edges into $A$. Formally, $\collapse{G}{A} = (V', E', r')$ such that $V' = \{A\} \cup (V' - A)$, $E' = \{e \in E \mid r(e) \not \subseteq A\}$ and two possible cases happen: for every $e \in E'$ either (1) $r'(e) = r(e)$ whenever $r(e) \cap A =\emptyset$, or (2) $r'(e) = \{v, A\}$ whenever $r(e) = \{v, v'\}$ with $v \notin A$ and $v' \in A$. We also define the graph $G_A = (A, E_A, r_A)$ such that $E_A$ and $r_A$ is restricted to edges in $A$, namely, $E_A = \{e \in E \mid r(e) \subseteq A\}$ and $r_A = r[E_A]$ where $r[E_A]$ is the function $r$ restricting the domain to $E_A$.

\begin{theorem}
	Let $G = (V,E)$ be a graph and $A \subseteq V$.  Then:
	$$
	\scen_{G}(A) \ = \ \scen_{\collapse{G}{A}}(A) +  |E_A|
	$$
\end{theorem}

\begin{proof}
	\cristian{Reescribir esta demostración bien y con la notación nueva de multigrafos.}
	
	First, it is clear that $\scen_{G(S)}(S)$ are just every subgraph of $G(S)$ that contains every node in $S$. This means that every edge in $E(S)$ could be added or removed to make a new subgraph. Thus, $$\scen_{G(S)}(S)= |\sgu_{G(S)}(S)| = 2^{|E(S)|}.$$
	
	On the other hand, let $G'$ be a subgraph of $G$ where every strongly connected component has at least one node from $S$. Then, it can be divided into two parts. The one that is purely contained in $G(S)$ and the one that only has edges outside of $S$. Then this is counted in $$\sum_{G'\in \sgu_{G(S)}(S)}\scen_{G\downarrow S}(x_S) = \scen_{G\downarrow S}{x_S}|\sgu_{G(S)}(S)|.$$
	
	This means that $$\scen_{G}(S)\leq \scen_{G\downarrow S}(x_S)|\sgu_{G(S)}(S)|.$$ 
	
	In the other direction, it is true that if we take an element from $\scen_{G\downarrow S}(x_S)|\sgu_{G(S)}(S)|$ there is a corresponding subgraph of $G$ where every strongly connected component has non empty intersection with $S$. Therefore, $$\scen_{G}(S) \geq \scen_{G\downarrow S}(x_S)|\sgu_{G\downarrow S}(x_S)|$$
	
	\textbf{Note:} Remember that $\scen_{G\downarrow S}(x_S) = |\sgc{G\downarrow S}{x_S}|$. Then $$\sum_{G'\in \sgu_{G(S)}(S)}\scen_{G\downarrow S}(x_S) = |\sgc{G\downarrow S}{x_S}||\sgu_{G(S)}(S)|.$$
\end{proof}

\cristian{Lo que sigue acá no se donde colocarlo ya que estaba inconcluso.}

This theorem shows that the extension for sets is reduced to compute the centrality of a node in a new graph.

Naturally, a more general notion appear when we take subgraphs as and argument for subgraph centrality.

\begin{definition}
	
	Let $G' = (V_{G'}, E_{G'}) \in \sgc(G)$ be an arbitrary connected subgraph of $G$. We define the centrality of $G'$ in $G$ as $$\scen_G(V_{G'},E_{G'}) = \log\left(|\{F \subseteq \sgc(G) \mid G' \in F\}|\right),$$
	
	which are all the subgraphs of $G$ that contains $G'$.
	

\end{definition}

The following definition is useful for some examples of subgraph centrality calculations.

\begin{definition}
	Let $G=(V,E)$ be a connected graph. We define the distance from a node $x$ in $V$ to an edge $e$ in $E$ as $$d_x(e) = \min_{u\in V, u \in e}\{d_G(x,u),d_G(u,x)\},$$
	where $d_G(x,u)$ is the usual geodesic distance between nodes.
\end{definition}

\begin{example}
	For a circuit of length $n\geq 3$, then $$arg\max_{S\subseteq V, |S| = 2} \scen_{C_n}(S) = \left\{0,\frac{n}{2}\right\}.$$
	
	This is, the maximum centrality for a set of size $2$ is reached when the nodes in the set $S$ are at distance $n/2$.
	
	\cristian{Este ejemplo estaba en otra sección antes y lo dejo acá para no perderlo.}
\end{example}

==> app-computeRoot.tex <==
We know that multiple centrality measures, are capable of defining a root for undirected trees. In this section we explore the problem of computing such roots for an arbitrary measure which enjoy the axioms from section~\ref{sec:Axioms}. Algorithm~\ref{Alg:alg2} essentially does this. For an arbitrary centrality measure $C$ satisfying every axiom from section~\ref{sec:Axioms} and tree $T$, this algorithm find the most central node of $T$. Before explaining the algorithm, we must proof the following theorem that ensure its correctness.


\begin{theorem}\label{Th:theoalg}
	Let $\preceq$ be a ranking which satisfies monotonicity, leaf beats parent and rank monotonicity axioms. Let $T$ be any tree and $u,v$ in $V(T)$, where $\pi_{uv}:= u = w_1w_2...w_n=v$ is the unique path connecting $u$ to $v$ in $T$.  Now, if $(u, T-\{u,w_2\})\preceq C(v,T-\{v,w_{n-1}\})$ then $(u, T) \preceq (w_2,T)$.
\end{theorem}

\begin{proof}
	In first place, by rank monotonicity we know that 
	\begin{equation}\label{eq:eq1}
		(u, T) \preceq (w_2,T) \text{ if and only if } (u, T - \{u,w_2\}) \preceq (w_2,T - \{u,w_2\}).
		\end{equation}
In consequence, we just have to prove the second inequality in equation~\ref{eq:eq1}. Now, by monotonicity we know that 
\begin{equation}\label{eq:eq2}
	(w_2, T - \{u,w_2\}) \succeq (w_2, T-\{\{w_2, z\}\mid z\in (N(w_2)\backslash \{w_3\})\}). 
\end{equation}


Notice that $w_2$ in the tree $T-\{\{w_2, z\}\mid z\in (N(w_2)\backslash \{w_3\})\}$ is a leaf hanging from $w_3$. Therefore, by leaf beat parent axiom we know that 
\begin{equation}\label{eq:eq3}
	(w_2, T-\{\{w_2, z\}\mid z\in (N(w_2)\backslash \{w_3\})\}) \succ (w_3, T -\{w_3, w_2\}).
\end{equation}
Now, combining equation~\ref{eq:eq2} and \ref{eq:eq3} we have that 
\begin{equation}
	(w_2, T - \{u,w_2\}) \succeq (w_3, T -\{w_3, w_2\}).
\end{equation}

We can repeat this process until we reach $w_{n}$ and then 

\begin{equation}\label{eq:eq4}
	(w_2, T - \{u,w_2\}) \succeq (w_{n}, T-\{w_{n-1},v\}).
\end{equation}

Finally, by hypothesis we know that  $(v, T-\{w_{n-1},v\}) \succeq (u, T-\{u,w_2\})$. Thus, this fact plus equation~\ref{eq:eq4} implies that

\begin{equation}
	(w_2, T - \{u,w_2\}) \succeq (u, T-\{u,w_2\}).
\end{equation}

\end{proof}

%\begin{algorithm}
%	\SetAlgoLined
%	\SetKwFor{While}{while}{}{end while}
%	\KwIn{A tree $T$ and a ranking $C$.}
%	\KwOut{The most central node of $T$ according to $C$.}
%	%initialization\;
%	
%	\SetKwFunction{Root}{Root}
%	\SetKwProg{Fn}{Function}{:}{}
%	\Fn{\Root{$T, C$}}{
%		
%		$P \gets \emptyset$\;
%		$U \gets V(T)$\;
%		$M \gets \emptyset$\;
%		
%		\ForEach{$v$ leaf of $T$}{
%			$p \gets C(\{v\}, (\{v\}, \emptyset))$\;
%			$P \gets \pinsert(P, v, p)$\;
%			$U \gets U \setminus \{v\}$\;
%		}
%		\While{$|U|>1$}{
%			\ForEach{$v \in U$}{
%				\If{$|N_T(v) \cap M| \geq |N_T(v)|-1$}{
%					$U \gets U \setminus \{v\}$\;
%					$p \gets C(v, T[\{v\} \cup (N_T(v) \cap M)])$\;
%					$P \gets \pinsert(P, v, p)$\;
%				}
%			}
%			$u \gets \pfind(P)$\;
%			$M \gets M \cup \{u\}$\;
%			$P \gets \pdelete(P)$\;
%		}
%		\KwRet $v \in U$\;
%	}
%	
%	\caption{Computing the root of a tree.}
%	\label{Alg:alg2}
%\end{algorithm}
\bigskip


In order to understand the notation from algorithm~\ref{Alg:alg2}, the set $U$ contain unmarked nodes. The centrality value for each node in $U$ has not been computed yet because there are nodes in $V$ with lower centrality value in its subtree. On the contrary, set $M$ contains all the nodes that have a centrality value that is lower than other node in the graph. Therefore, the most central node will never be in $M$. On the other hand, we use a priority queue $P$ where the functions $\text{find-min}(P)$ gets the minimum element in $P$, $\text{delete-min}(P)$ output a new priority queue without the minimum element in $P$ and $\text{insert}(P,v,p)$ generates a new priority queue with the same elements in $P$ plus element $v$ with value $p$. Finally, for a tree $T$, the notation $T[S]$ for a set of nodes $S\subseteq V(T)$ represent the induced graph by $S$ in $T$. Therefore, $T[\{v\} \cup (N_T(v) \cap M)]$ represent the tree generated by $v$ and every neighbour of $v$ that has already been marked.

\smallskip
Algorithm~\ref{Alg:alg2} explanation goes as follow. In first place, because of the rooting tree property, we know that leaves can never be the most central nodes. Then, algorithm~\ref{Alg:alg2} set values to every leaf as their centrality value as isolated nodes and then add them to $P$. The priority queue $P$ is an intermediate data structure that allows us to store the candidates to be marked. In the second while loop, the algorithm goes through every unmarked node such that at most one neighbour is not marked and add them to $P$. Then, the node with lowest centrality value in $P$ is added to $M$. By theorem~\ref{Th:theoalg} we know that the node with lowest centrality value in its subtree will always have a neighbour with greater centrality value in the whole tree. This implies that the most central node can never be added to $M$. Clearly, in each iteration we remove one node from $U$ and add it to $M$. Finally, where $|U| = 2$, the nodes in $U$ are two connected nodes. Therefore, by ranked monotonicity, the most central node will not be marked because we compare both centrality values in the respective subtree. Which concludes that when $|U|=1$ the unique node in $U$ must be the most central node in $T$ according to $C$.


\subsection{Bounds for roots}

In this section we give important bounds for the roots in any tree with a fixed amount of nodes $n \geq 1$. Essentially, the importance of any root in a tree with $n$ nodes is bounded, in the lower side, by the importance of the least relevant node in a line with $n$ nodes, the extreme. On the other side, the importance of a root in any tree with $n$ vertices is upper bounded by the importance of the most central node in a star tree with $n$ nodes. The following theorem states a sufficient condition in order to have such bounds.

\begin{theorem}\label{theo:bounds}
	Let $\preceq$ be any ranking satisfying the close under isomorphism, strong monotonicity, rank monotonicity, leaf beats parent and leaf monotonicity axioms. Then, for every $n\geq 1$, if $T$ is a tree such that $|V(T)| = n$ and $v$ is a node in $T$, then $$ (0, L_{n-1})\preceq 
	(v, T) \preceq (0, S_n).$$
\end{theorem}

\begin{proof}
The proof goes by strong induction on $n$. For $n=1$ and $n = 2$ this is trivial since the line and the star graphs are the same. By close under isomorphism we know any tree with such structure will have the same centrality value. Now, for $n > 1$, we have two cases depending if $v$ is a leaf or not. If $v$ is a leaf in $T$ hanging from a node $u$, then $(0, L_{n-2})\preceq (u, T-\{v\}) \preceq (0, S_{n-1})$ by hypothesis. Then, by leaf monotonicity, $(0, L_{n-1}) \preceq (v, T)$ and $(v, T)\preceq (0, S_{n})$. In the second case, if $v$ is not a leaf in $T$, then $v$ is a cut vertex such that $T_1 \cup T_2 = T$ and $V(T_1)\cap V(T_2) = \{v\}$. Therefore, $|V(T_1)| + |V(T_2)| = n + 1$ but $|V(T_1)| < n$ and $|V(T_2)| < n$. Without loss of generality we can assume that $(v, T_1) \preceq (v, T_2)$. Now, by strong monotonicity plus the induction hypothesis and close under isomorphism we can conclude that $(v, T_1\cup T_2) \preceq (v, T_1\cup L_{|V(T_2)|})$ since $(v, T_2) \preceq (0, L_{|V(T_2)|})$ (here we assume $v$ is the extreme of a line with $|V(T_2)|$ nodes). Using the same argument we know that $(v, T_1) \preceq (v, L_{|V(T_1)|})$ and therefore $(v, T_1\cup L_{|V(T_2)|}) \preceq (v, L_{|V(T_1)|}\cup L_{V(T_2)}) \preceq  (0, L_{n})$ since the rooting tree property implies the extreme of a line is always less central than any node in between. In the other hand, we can use a similar argument. If $(v, T_1) \preceq (v, T_2)$ then $(v, T_1 \cup T_2) \preceq (v, T_2\cup S_{|V(T_1)|})$ using the axioms and induction hypothesis. Again, we can use the same argument to show that $(v, T_2\cup S_{|V(T_1)|}) \preceq (v, S_{|V(T_2)|}\cup S_{|V(T_1)|}) \equiv (0, S_{n})$ by close under isomorphism.
 
\end{proof}

==> app-functions.tex <==


%\subsubsection{Cut vertex function}
Now that we know when a ranking can root trees, it is essential to have a method to find such rankings. For that purpose, we introduce a set of centrality measures which natural ranking can root trees. Such measures are defined by the way a it grows and behaves within trees using recursive functions. Some measures as allsubgraphs centrality and counting subgraphs enjoy this structure. In both cases, there exists a cut vertex function that define the value of a cut vertex depending on the different components it is cutting and a leaf function which tells you what is the importance of a leaf depending on its parent value. To generalize this idea, we will look for general functions that explain the way a centrality measure can be obtained.

\smallskip
\textbf{Cut-vertex function} $F:\mathbb{R}\times\mathbb{R} \to\mathbb{R}$ is a cut vertex function if it is commutative i.e $F(a,b) = F(b,a)$, associative i.e $F(a,F(b,c)) = F(F(a,b), c)$, $F$ has an identity i.e there exists $k\in \mathbb{R}$ such that for every $a$ in $\mathbb{R}$ then $F(a,k) = a$ and monotonic i.e for every $a \geq k$ and $b > k$  $\implies a < F(a,b)$. Some examples of a cut-vertex function can be the usual multiplication or addition in $\mathbb{R}$. For simplicity of notation we will use $F(a,b)= a\ast b$ indistinctly when the function $F$ is clear.


\smallskip
Now it is necessary to stablish a function that tells us how centrality is transferred to a leaf from its parent. In other words, when a new leaf is added, we assume there is a value this leaf is receiving depending on its parent importance.

\smallskip
\textbf{Leaf function.} Given a cut-vertex function $F$ with identity $k$, we call $H:\mathbb{R}\to\mathbb{R}$ a leaf function for $F$ if for every $a \geq k$ then $a < H(a)$.

\smallskip
For a cut-vertex function $F$ with identity $k$ and a leaf function $H$ there is a unique centrality measure $C_{F,H}$ defined recursively as follow. For a node $v$ then $C_{F,H}(v, (\{v\},\emptyset)) = k$. Then, for a tree $T$ and a leaf $u$ in $V(T)$ with parent $v$, then $C_{F,H}(u, T) = H(C_{F,H}(v,T-\{u\}))$. Finally, for trees $T_1,T_2$ such that $V(T_1)\cap V(T_2) = \{v\}$, then $C(v,T_1\cup T_2) = F(C_{F,H}(v,T_1), C_{F,H}(v, T_2)).$ The centrality measure $C_{F,H}$ is well defined because of the facts that $F$ is commutative, associative and $k$ is the identity. Therefore, it does not matter how we decompose the different components for a cut-vertex $v$, we will always get the same value for $C_{F,H}$.

\smallskip
Now, since $C_{F,H}$ is completely defined by $F$ and $H$, the axioms from section~\ref{sec:Axioms} can be translated into properties over $F$ and $H$. We present such characterizations as follow.

\begin{lemma}[Monotonicity]
The centrality measure $C_{F,H}$ always enjoy the monotonicity axiom.
\end{lemma}
\begin{proof}
	If $T_1,T_2$ are two trees such that $V(T_1)\cap V(T_2) = \{v\}$ then by definition of the cut-vertex function $F$, if $T_2 = (\{v\},\emptyset)$ then $C_{F,H}(v, T_2) = k$. Therefore, $C_{F,H}(v, T_1) = C_{H,F}(v,T_1)\ast k$. In the other hand, if $T_1$ and $T_2$ are not isolated nodes, then $C_{F,H}(v, T_i)>k$ because $H$ and $F$ will always increase the value from an isolated vertex. Therefore, $C_{F,H}(v, T_1\cup T_2) = F(C_{F,H}(v, T_1),C_{F,H}(v, T_2)) > F(C_{F,H}(v, T_1), k) = C_{F,H}(v, T_1)$ because $C_{F,H}(v, T_2) > k$ and $F$ is monotonic.
\end{proof}

\begin{lemma}[Leaf beat parent]\label{lemma:LFBfunction}
	The centrality measure $C_{F,H}$ always enjoy the leaf beat parent axiom.
\end{lemma}

\begin{proof}
	This comes directly from the definition of the leaf function $H$. Therefore, if $u$ is a leaf hanging from $v$ in $T$, then $C(u, T) = H(C(v, T-\{u\}) > C(v, T-\{u\})$.
\end{proof}

\begin{lemma}[Rank monotonicity]\label{lemma:RankMonfunct}
	The centrality measure $C_{F,H}$ enjoys the ranking monotonicity axiom if and only if $a\leq b \iff F(a, H(b)) \leq F(H(a), b)$ for every $a,b \in \mathbb{R}$.
\end{lemma}

\begin{proof}
	This is just the definition of the ranking monotonicity axiom.
\end{proof}
%$T_1$ and $T_2$ are two disjoint trees where $V(T_1)\cap V(T_2) = \{v\}$, then $$C(v, T_1\cup T_2) = F(C(v,T_1), C(v,T_2)).$$


%Directly from this definition we can conclude that $F$ must be commutative i.e $F(C(v,T_1), C(v,T_2)) = F(C(v,T_2), C(v,T_1))$  and associative i.e $F(F(C(v,T_1),C(v,T_2)), C(v,T_3)) = F(C(v,T_1),F(C(v,T_2), C(v,T_3)))$ since the centrality of $v$ is uniquely defined. For this reason from now on we will simplify our notation as $F(a,b,c) = F(F(a,b),c)= F(a,F(b,c))$.

From the previous definition it is easy to see that if $F=\times$ is the usual multiplication and $H(a) = a+1$ then $C_{\times,H}$ is equal to counting subgraphs. In the other hand, when $F=+$ is the addition in $\mathbb{R}$ and $H(a) = \log(1+2^{a})$ then $C_{+, H}$ is equal to all subgraphs centrality.

%\begin{definition}
%	For a cut-vertex function $F$ we say that it is increasing if for every cut vertex $v$, then $C(v,T_1) \leq F(C(v,T_1),C(v,T_2))$ and $C(v,T_1) = F(C(v,T_1),C(v,T_2))$ iff $T_2$ is an isolated vertex.	
%\end{definition}
%In other words we want that this function $F$ increase whenever we compute the centrality of a cut vertex of two disjoint trees that are not isolated vertices. Therefore, we can translate the increasing property as 
%\begin{equation}\label{eq:identity}
%\forall a, a = F(k,a) = F(a,k)
%\end{equation}
%\begin{equation}
%\forall a\forall b, (a\not=k \wedge b\not= k) \implies (a< F(a,b)\wedge b < F(a,b))
%\end{equation}
%
%Finally, equation~\ref{eq:identity} means that $k$ is an identity for $F(\cdot,\cdot)$. Combining this with the commutative and associative properties it implies that $(k,F)$ forms a commutative monoid in $R^{\geq k}$. For this reason, from now on we denote 
%
%\begin{eqnarray}
%a\ast b :=& F(a,b)\\
%\mathds{1} :=& k
%\end{eqnarray}
%where $(\mathbb{R}^{\geq k}, \ast, \mathds{1})$ is a commutative monoid and $a<a\ast b$ when $b>\mathds{1}$.
%
%%\subsubsection{Leaf adition function}
%
%
%
%\smallskip
%\ax{7}{leaf function} Let $C$ be a centrality measure and $T$ a tree such that $u$ is not a node from $T$. We say that $C$ has the Leaf adition function property if there exists a function $H_C:\mathbb{R}^{+}\to \mathbb{R}^{+}$ such that $C(u, T + \{u,v\}) = H_C(C(v, T))$.
%\smallskip
%
%For example, in all subgraphs centrality when $u$ is not in $V(T)$ we have that $\Acen(v, T)= \log(\Subg(v,T))\implies k(\Acen(v,T)) = 2^{\Acen(v,T)} = \Subg(v,T)$. Therefore, for allsubgraphs centrality $\Acen(u, T+\{u,v\}) = \log(1+k(\Acen(v,T))) = H_{\Asg}(\Acen(v,T))$. On the other hand, for counting subgraphs we have $\Subg(u,T +\{u,v\}) = 1 + \Subg(v,T) = H_{\Subg}(\Subg(v,T))$. Finally, we can define the edges centrality as $C_{|E|}(v,G) = |E(G)|$. In this case, we have $C_{|E|}(u,T + \{u,v\}) = 1 + C_{|E|}(v,T) = H_{|E|}(C_{|E|}(v,T))$. Therefore, this proves that isolated constant, Leaf adition function and cut-vertex function are not very informative by themselves because very useless centralities as counting edges have the same function $H$ as another more complex as counting subgraphs. For this reason we want to ask for more restriction to the functions $H$ and $\ast$. In first place, $H$ must be a strictly increasing function since the centrality of a parent should be at least completely transferred to their son.
%
%\begin{definition}
%	If $C$ is a centrality measure satisfying Leaf adition function. We say that $H_C$ is strictly increasing if $C(v,T)< H_C(C(v,T)) = C(u,T + \{u,v\})$ for a node $u\not\in V(T)$.
%\end{definition}
%
%%\begin{definition}
%%	If $C$ is a centrality measure satisfying Leaf adition function and cut-vertex function. We say that $H_C$ is bounded by $F_C$ if $H_C(C(u, T-v)) \leq H_C(k)\ast C(u, T-v)$ for a leaf $v$ hanging from $u$.
%%\end{definition}
%
%%In other words, if a centrality measure satisfies both definition. The importance of a leaf must be strictly greater than his parent importance before adding it to the tree. Simultaneously, the centrality of its parent should be greater than his after we add the leaf. 
%
%This property can be translated as $\forall a, a < H_C(a)$. The intuition behind strictly increasing functions is based on how parents pass their centrality over descendants. It is natural to think that every child it least as important as their parents. However, we ask for strictly increasing because we want that centrality actually grow for more complex structures. 
%
%On the other hand, to have a more interesting set of properties we want that $\ast$ respect the centrality asymmetry when connecting two disjoint components.
%
%\smallskip
%If a centrality measure preserve asymmetry it is equivalent to say that over $(\mathbb{R}^{\geq k},\mathds{1},\ast, H), 
%$ $$\forall a,b, \text{ if } a\leq b \iff a\ast H(b)\leq b\ast H(a).$$
%This particular property is where counting edges fails. When we connect two trees, every node in the new graph has the same centrality value and therefore, it does not preserve the asymmetry.
%
%Finally, we want that $\ast$ preserve order. This is a much stronger property but has a lot of intuition in the context of trees.
%
%\smallskip
%Preserving order can be translated to $\forall a,b,c, a < b\iff a\ast c < b \ast c$ which means that $(\mathbb{R}^{\geq k}, \ast, \mathds{1}, \leq)$ is and ordered commutative monoid.

\subsection{$\alpha,\beta$ leaf functions}


We define the leaf function $H_{\alpha,\beta}(x) = \alpha x + \beta$ for $\alpha,\beta \in \mathbb{R}$. Then, we will use $a\ast b = a\times b$ the usual multiplication in $\mathbb{R}$ as the cut-vertex function. Which means we have the identity $k = 1$. However, it is important to state which values of $\alpha$ and $\beta$ define a proper leaf function i.e for every $a \geq k$, then $H_{\alpha,\beta}(a) > a$. If $a$ is any value greater than $k = 1$, then $H_{\alpha,\beta}(a) = \alpha a +  \beta > a$ if and only if $\beta > a(1-\alpha)$. Then, if $1-\alpha < 0$ this inequality holds if and only if $\displaystyle\frac{\beta}{1-\alpha} < a$ which is always the case when $\beta >0$ since $a \geq k = 1$. On the other hand, if $(1-\alpha) > 0$, the property holds iff $\displaystyle\frac{\beta}{1-\alpha} > a$. Thus, there could exists values where this inequality is not true since the cut vertex function $\times$ is not bounded. In consequence, when we use $\times$ as the cut vertex function, we just will allow values $\alpha \geq 1$ and $\beta > 0$. By lemma~\ref{lemma:LFBfunction} we know that the measure $C_{\times, H_{\alpha,\beta}} =  C_{\alpha,\beta}$ will satisfy the leaf beats parent axiom. In the same way, this measure enjoy the monotonicity axiom since the usual multiplication is monotonic. Finally, for $a,b \geq 1$ we have that $H_{\alpha,\beta}(a)\times b = (\alpha a + \beta)b \geq H_{\alpha,\beta}(b)\times a = (\alpha b + \beta)a$ if and only if $a \geq b$ and therefore, $C_{\alpha,\beta}$ satisfies every axiom.

\smallskip
It can be seen in figure~\ref{fig:example1} where graph $G_1^n$ is the star with $n$ nodes while $G_2^n$ is an extension with $n/2$ nodes surrounding the center. For any centrality $C$ defined by functions $H_C$ and $F_{C}$, we have that $C(1, G_1^n) = H_C(H_C(k_C)^{n-1})$ while $C(0,G_2^n) = H_C(H_C(k_C))^{n/2}$. In our example, $C_{\alpha,\beta}(1,G_1^n)= \alpha((\alpha+\beta)^{n-1}) + \beta$ and $C_{\alpha,\beta}(0,G_2^n)=(\alpha(\alpha+\beta)+\beta)^{n/2}$. We know that counting subgraphs is defined by $\alpha = 1$ and $\beta = 1$. Then, $C_{1,1}(1,G_1^n) = 2^{n-1}+1$ and $C_{1,1}(0,G_2^n) =3^{n/2}$. Which means that for $n\leq 4, C_{1,1}(0,G_2^n) = 3^{n/2}\geq 2^{n-1}+1 = C_{1,1}(0,G_2^n)$.  Therefore, the question is: for which $\alpha$ and $\beta$ exists $n\leq 4$ such that $C_{\alpha,\beta}(1, G_1^n) > C_{\alpha,\beta}(0, G_2^n)$?. This would imply, by ranking monotonicity axiom, that $C_{\alpha,\beta}$ will differ with counting subgraphs ranking between node $0$ and node $1$ in the graph $G_1^n + G_2^n + \{0,1\}$. This question will remain open in the general case but we could prove that for $\alpha = 2, \beta=1$ and $n =4$ ranking from $C_{\alpha,\beta}$ differ with counting subgraphs.
\begin{figure}[]
	\centering
	
	\begin{tikzpicture}[scale=0.07,text width=5mm]
		\node (b) at (-20,10)  {\Large $G_1^n$};
		\node (a) at (0,0) [ble, thick] {\textbf{0}};	
		
		\foreach \a in {1,2,...,6}{
			\draw (360*\a/8: 12cm) node[ble] (\a) {\a};
			\draw[-] (a) to (\a);
		}
		
		\draw (7*360/8: 12cm) node[ble, draw=white] (ldots) {\large $\cdots$};
		\draw[-] (a) to (ldots);
		
		\draw (8*360/8: 12cm) node[ble] (n) {n};
		\draw[-] (a) to (n);
		
		\begin{scope}[xshift = 50cm]
			\node (b) at (30,10)  {\Large $G_2^{n}$};
			\node (a) at (0,0) [ble, thick] {\textbf{0}};	
			
			\foreach \a in {1,2,...,6}{
				\draw (360*\a/8: 12cm) node[ble] (\a) {};
				\draw[-] (a) to (\a);
			}
			
			\foreach \a in {1,2,...,6}{
				%\pgfmathtruncatemacro\mymacro{\a+6}
				\draw (360*\a/8: 24cm) node[ble] (2\a) {\a};
				\draw[-] (2\a) to (\a);
			}
			
			\draw (7*360/8: 12cm) node[ble, draw=white] (ldots) {\large $\cdots$};
			
			\draw (8*360/8: 12cm) node[ble] (n) {};
			\draw[-] (a) to (n);
			
			
			\draw (8*360/8: 24cm) node[ble] (n2) {$n/2$};
			\draw[-] (n2) to (n);
		\end{scope}
	\end{tikzpicture}

	\caption{Example for $H_{\alpha,\beta}$.}
	\label{fig:example1}
\end{figure}

These functions show that there are infinitely many centrality measures with potentially different rankings which are able to root trees. Therefore, more study cases arise to spot the differences between these measures for different $\alpha$ and $\beta$ values. In first place, the center of a star graph with $n$ nodes ($S_n$), is the most connected node in a tree with $n$ nodes. In the other hand, the extreme of a line with $m$ nodes ($L_m$) is the less connected node in the most sparse tree with $m$ nodes. Then, if $v$ is the center $S_n$ then $C_{\alpha,\beta}(v,S_n)=(\alpha+\beta)^{n}$. While if $u$ is the extreme of $L_m$ then $C_{\alpha,\beta}(u,L_m) = H_{\alpha,\beta}^{m}(k)=\sum_{i=0}^{m-1}\alpha^{i}\beta + \alpha^{m}$. For example, if we fix $\beta=1$, for which values of $\alpha,n$ and $m$ then $(\alpha+1)^{n}\leq \sum_{i=0}^{m}\alpha^{m}$? In such case the extreme of a line would as central as the center of a star which is an unexpected behaviour in general. If $\alpha>1$ we know that $\sum_{i=0}^{m}\alpha^{m}=\displaystyle\frac{\alpha(\alpha^{m}-1)}{\alpha-1}\in O(\alpha^{m})$. Therefore, for $\alpha>1$ we just need a lineal amount of nodes in the line $L_m$ in order to equal the order of centrality reached by the center of a star $S_n$. In the other side, if $\alpha<1$ then $\sum_{i=0}^{m}\alpha^{m} = \displaystyle\frac{\alpha(1-\alpha^{m})}{1-\alpha}\leq \displaystyle\frac{1}{1-\alpha}$ and therefore the centrality value of the extreme in a line with $m$ nodes is upper bounded. At the same time, the value of the center node from a star $S_n$ is increasing with respect to $n$. Which means that there exists $n>1$ such that $C_{\alpha,\beta}(v, S_n)>C_{\alpha,\beta}(u,L_m)$ for every $m>1$. Finally, the case where $\alpha=1$ is left. In this case $\sum_{i=0}^{m}\alpha^{m}=m$, which means that we will need exponentially more nodes in the line than in the star in order to have more value in the extreme than on the center.

\subsection{$\gamma$ cut vertex functions}

In the previous section, $\alpha$ and $\beta$ leaf functions were analysed assuming the usual multiplication as the cut vertex function. Now, for $\gamma > 0$, we define the cut vertex function $F_{\gamma}(a,b)= \displaystyle\frac{a\times b}{\gamma}$. Therefore, for a given $\gamma$ the identity for $F_{\gamma}$ is $k = \gamma$. We wonder now, how the ranking defined by $C_{F_{\gamma}, H_{\alpha,\beta}} = C_{\alpha, \beta,\gamma}$ differ for different values of $\alpha, \beta$ and $\gamma$. In first place, we must state which values are allowed in order to define a proper rooting centrality measure i.e a centrality enjoying every axiom. In first place, we want that $H_{\alpha,\beta}(a) > a$ for every $a\geq \gamma$. Similarly to the previous section, this is true if and only if $\beta > a(1-\alpha)$. Now, if $(1-\alpha) < 0$ then this inequality holds if and only if $\displaystyle\frac{\beta}{1 - \alpha} < a$, which again is always the case since $a \geq \gamma > 0$. In the case that $(1-\alpha) > 0$ the inequality holds whenever $\displaystyle\frac{\beta}{1 - \alpha} > a$. In this case, since we want a monotonic cut-vertex function, the inequality can not hold for every $a$. Therefore, we will only accept values of $\alpha \geq 1$, $\beta > 0$ and $\gamma > 0$. In the case of ranking monotonicity, it is easy to see that the inequality of lemma~\ref{lemma:RankMonfunct} does not depend on $\gamma$. Finally, monotonicity follows from the fact that $a < F_{\gamma}(a,b)$ for every $b \geq \gamma$.

\smallskip
Certainly, it is not an easy task to analyse the behaviour of $C_{\alpha,\beta,\gamma}$ without fixing some values in $\alpha$ and $\beta$. The same analysis for graphs $G_1^{n}$ and $G_2^n$ in figure~\ref{fig:example1} can be done in this case. We have that $C_{\alpha,\beta,\gamma}(1,G_1^{n}) = H_{\alpha,\beta}\left(\displaystyle\frac{H_{\alpha,\beta}(\gamma)^{n-1}}{\gamma^{n-2}}\right) = \alpha\left(\displaystyle\frac{(\alpha\gamma + \beta)^{n-1}}{\gamma^{n-2}}\right) + \beta.$ In the other hand, $C_{\alpha,\beta,\gamma}(0, G_2^n)= \displaystyle\frac{H(H(\gamma))^{n/2}}{\gamma^{n/2 - 1}} = \displaystyle\frac{(\alpha(\alpha\gamma + \beta) + \beta)^{n/2}}{\gamma^{n/2 - 1}}$. Now, if we fix $\alpha = 1, \beta = 1$ and $n = 4$ we have that for $\gamma = 0.5$ then $C_{\alpha,\beta, \gamma}(1, G_1^{4}) = 13,5$ while $C_{\alpha, \beta,\gamma}(0, G_2^{4}) = 12,5$. However, for $\gamma = 1$, then $C_{\alpha,\beta, \gamma}(1, G_1^{4}) = 8$ and $C_{\alpha, \beta,\gamma}(0, G_2^{4}) = 9$. Therefore, the rankings interchange for these different values of $\gamma$.

\smallskip
It is interesting to study how $C_{\alpha,\beta,\gamma}$ differentiates between a star (the most central tree) and the line (the most sparse tree). As we did in the previous section, for a star with $n$ nodes sorrounding the center $0$, we have the expression $C_{\alpha,\beta,\gamma}(0, S_n) = \displaystyle\frac{H_{\alpha,\beta}(\gamma)^{n}}{\gamma^{n-1}} = \displaystyle\frac{(\alpha \gamma +   \beta)^n}{\gamma^{n-1}}$. On the other hand, for the extreme of the line with $n$ nodes we have that $C_{\alpha,\beta,\gamma} (0, L_n) = H^{n}(\gamma) = \alpha H^{n-1}(\gamma) + \beta = ... = \alpha^{n}\gamma + \sum_{i=0}^{n-1}\alpha^i\beta$. In this case, when $\gamma \to \infty$ and $n$ is fixed, both values get closer to each other. In other words, $\lim\limits_{\gamma \to \infty} C_{\alpha,\beta,\gamma}(0,S_{n-1}) - C_{\alpha,\beta,\gamma}(0,L_n) = 0$. However, since $F_{\gamma}$ is monotone, whenever $n_1 > n_2$ then $C_{\alpha,\beta,\gamma}(0, S_{n_1})> C_{\alpha,\beta,\gamma}(0, S_{n_2})$. At the same time, theorem~\ref{theo:bounds} implies that every graph with $n$ nodes has the same importance for $C_{\alpha,\beta,\gamma}$ as $\gamma\to \infty$. This implies that when $\gamma \to \infty$ and $\alpha = \beta = 1$, then $C_{\alpha,\beta,\gamma}$ get closer to a measure which only differentiate between graphs with different amount of nodes. Essentially how closeness assign the most important node in a graph. 


==> app-generalization.tex <==
In this section we will seek for a collection of general properties that captures the set of rankings that are able to decide the root of a tree.
We start by introducing the definition of a root in a tree $T$ according to a ranking $\preceq$.



\smallskip

\begin{definition}[Rooting-tree property]
	We say that a centrality ranking $\preceq$ has the \emph{rooting-tree property} if for every tree $T$, the set of most important vertices:
	$$
	\roots(T) \ = \ \{v\in V(T) \mid \forall u\in V(T).\,  u \preceq v \}
	$$ 
	is connected in $T$. Moreover, for any $v \in \roots(T)$ and $u \not= v$, if $\pi_{vu} = v_0 v_1...v_n$ is the unique path from $v$ to $u$ in $T$, then $(v_{i+1}, T)\preceq (v_i, T)$ for every $i\in\{0,...,n-1\}$.
\end{definition}

The intuition behind this definition is based on the three principles. First, the most important node given by the ranking should be declared as the root of the tree. Second, if there are several most important nodes (i.e., they are ranked the same), then they must be connected since the root of a tree must be one source of importance. Last, regarding nodes that are not the root, we expect that the importance from the root through branches should decrease. In other words, the closer to the root a node is, the more important it is. Note that, given that $T$ is a tree and $\roots(T)$ must be connected, then $|\roots(T)| \leq 2$. For the case when $|\roots(T)| = 2$, we are assuming that the edge between the two most important nodes works as the root of the tree. 

Next, we show that a subset of the axioms implies the rooting tree property of a ranking. 

\begin{theorem} \label{Th:Theorem3_simpler}
	Suppose that $\preceq$ is a tree centrality ranking that satisfies closed under isomorphism, weak monotonicity, and rank monotonicity axioms. Then the following are equivalent:
	\begin{itemize}
		\item[(i)] $\preceq$ satisfies the leaf-beats-parent axiom.
		\item[(ii)] $\preceq$ satisfies the rooting-tree property. 
	\end{itemize}
\end{theorem}

\begin{proof}. 
We start by showing that stronger property that implies the rooting-tree property. We say that $\preceq$ has the \emph{at-most-one-parent} property if for every tree $T$ and node $v\in V(T)$ there exists at most one $u\in N_T(v)$ such that $(v,T) \preceq (u,T)$. We prove the following claim:
\begin{claim}\label{claim:AMOProot}
If a tree centrality ranking $\preceq$ enjoys the at-most-one-parent property then $\preceq$ satisfies the rooting-trees property.
\end{claim}

To show this claim, suppose that $\preceq$ enjoys the at-most-one-parent property. Let $v \in \roots(T)$ and take any node $u \in V(T)$. We first prove that if $\pi:=v = v_0...v_{n}=u$ is the unique path connecting $v$ to $u$, then $(v_{i+1}, T) \preceq (v_i, T)$ for every $i < n$. It is clear that $(v_1, T) \preceq (v_{0}, T)$ since $v_0 = v$ is in $\roots(T)$. Then, by induction over $i \geq 1$ we can conclude that $(v_{i+1}, T) \preceq (v_{i}, T)$ because $(v_{i}, T) \preceq (v_{i-1}, T)$ and $v_{i}$ can not have two neighbors with more importance than him.

For finishing the prove of the claim, it remains to show that the set $\roots(T)$ are connected in $T$. Consider a tree $T$ and $u,v\in V(T)$ such that $u\not= v$ and $\{u,v\}\subseteq\roots(T)$. By contradiction, suppose that $\{u,v\}\notin E(T)$, then there must be a path $\pi:=u = v_1...v_n=v$ connecting $u$ and $v$ such that $n>2$. Since $u$ and $v$ have the same importance, by the previous paragraph and the transitivity of $\preceq$, we know that $(u,T)\equiv(v_2,T) \equiv ... \equiv (v,T)$. This contradicts at-most-one-parent because every $v_i$ for $i\in\{2,...,n-1\}$ have at least two neighbors with more or equal importance than him. 

We use the claim for proving the equivalence between (i) and (ii). For this, assume that $\preceq$ satisfies closed under isomorphism, weak monotonicity, and rank monotonicity axioms.
\smallskip

\noindent (i) $\Rightarrow$ (ii): Suppose that $\preceq$ also satisfies the leaf-beats-parent axiom. By the previous claim it is enough to prove the at-most-one-parent property. 
Fix an arbitrary tree $T$, node $v$ and let $u,w$ be two arbitrary neighbors of $v$ in tree $T$.
By removing edges $\{u,v\}$ and $\{v,w\}$ we get a decomposition of $T$ into three trees, $T_u, T_v, T_w$ containing $u,v,w$, respectively, such that
\[ T = (T_v \cup T_u \cup T_w)+ \{u,v\} + \{v,w\}. \]
Without loss of generality assume $(w,T_w) \preceq (u,T_u)$.
From leaf-beats-parent we have $(u,T_u) \prec (v, T_u + \{u,v\})$ and using weak monotonicity we get $(u,T_u) \prec (v, (T_u + \{u,v\}) \cup T_v)$.
Based on our assumption $(w,T_w) \preceq (u,T_u)$, we conclude  $(w,T_w) \prec (v, (T_u + \{u,v\}) \cup T_v)$.
This, combined with rank-monotonicity, implies that $(w,T) \prec (v,T)$.
Hence, we just proved that out of every two neighbors at least one has smaller centrality than $v$ which implies the thesis.

\smallskip

\noindent (ii) $\Rightarrow$ (i):
Assume $\preceq$ violates leaf-beats-parent. 
We will show that it also violates at-most-one-parent.
Let $T$ be a tree, $u$ be a node in $T$ and $v \notin V(T)$ such that $(v,T + \{u,v\}) \preceq (u,T)$, namely, leaf-beats-parent is not satisfied.
Take a second tree $T'$ isomorphic to $T$ such that $u'$ corresponds to $u$.
From closed under isomorphism, we know that $(u',T') \equiv (u,T)$.
Let us construct a tree $T^*$ by adding $T'$ and edge $\{u',v\}$ to $T + \{u,v\}$: 
\[ T^* = (T + \{u,v\}) \cup (T' + \{v,u'\}). \]
From $(v,T + \{u,v\}) \preceq (u,T)$ and rank-monotonicity we get:
\[ (v,T^*) \preceq (u',T^*). \]
Analogously (or directly from closed under isomorphism) we get that $ (v,T^*) \preceq (u,T^*)$ which means at-most-one-parent axiom is not satisfied.	
\end{proof}

Theorem~\ref{Th:Theorem3_simpler} is our first result which relates all of the proposed axioms for rankings over trees. However, this set of axioms is not enough to characterize every ranking with the rooting property as can be seen in the following example.

\begin{example}
	The ranking $\preceq_{\textsc{Closeness}}$ roots trees but  does not enjoy the monotonicity and rank-monotonicity axioms.
\end{example}

\begin{example}
	The ranking $\preceq_{\textsc{Betweenness} }$ is not a rooting tree ranking.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/betNotRoot.png}
	\caption{Betweenness can not root.}
\end{figure}

\begin{example}
	The ranking $\preceq_{\textsc{Attachment}}$ is not a rooting tree ranking.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/AttachNotRoot.png}
	\caption{Attachment can not root.}
\end{figure}

\begin{example}
	The ranking $\preceq_{\textsc{Bonacich}}$ is not a rooting tree ranking for $a = 0.2$.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/AttachNotRoot.png}
	\caption{Bonacich can not root for $a = 0.2$.}
\end{figure}

\begin{example}
	The ranking $\preceq_{\textsc{Flow-Bet}}$ is not a rooting tree ranking.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/FlowBetNotRoot.png}
	\caption{Flow Betweenness can not root.}
\end{figure}

\begin{example}
	The ranking $\preceq_{\textsc{Decay}}$ is not a rooting tree ranking for $\alpha = 0.5$.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/DecayNotRoot.png}
	\caption{Decay can not root for $\alpha = 0.5$.}
\end{figure}

\begin{example}
	The ranking $\preceq_{\textsc{EV}}$ is not a rooting tree ranking.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/EigenVecNotRoot.png}
	\caption{EigenVector can not root.}
\end{figure}

\begin{example}
	The ranking $\preceq_{\textsc{PR}}$ is not a rooting tree ranking.
\end{example}

\begin{figure}[H]
	\centering
	\includegraphics[scale = 0.6]{../Figures/PageRankNotRoot.png}
	\caption{PageRank can not root.}
\end{figure}

The following table summarizes the rooting tree measures.

\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|}
		\hline
		Measure         & Can root? \\ \hline
		Closeness       & Yes       \\ \hline
		Betwenness      & No        \\ \hline
		PageRank        & No        \\ \hline
		Decay           & No        \\ \hline
		Attachment      & No        \\ \hline
		Eccentricity    & Yes       \\ \hline
		AllSubgraphs    & Yes       \\ \hline
		EigenVector     & No        \\ \hline
		Flow Betwenness & No        \\ \hline
		Bonacich        & No        \\ \hline
	\end{tabular}
	\caption{Summary of rooting tree measures.}
\end{table}


\subsection{Potential functions and rooting}

We have shown that rankings let us to compare importance between nodes. Now we introduce potential functions to give more structure to how importance behave.

\textbf{Potential functions.} A function $f:\mathcal{V}\times \mathcal{G}^{\mathcal{V}}\to \mathbb{R}$ is a potential function for a given ranking $\preceq$ if for every $(v_1, T_1)$ and $(v_2, T_2)$ such that $V(T_1)\cap V(T_2) = \emptyset$ then $(v_1, T_1\cup T_2\cup \{v_1,v_2\}) \preceq (v_2, T_1\cup T_2\cup \{v_1,v_2\})$ if and only if $f(v_1, T_1) \leq f(v_2, T_2)$.

\begin{example}
	For $\preceq_{\textsc{Closeness}}$, the function $f(v, T) = |V(T)|$ is a potential function.
\end{example}

Not every potential function will be equally important for us. We give now some restrictions over potential functions that will be useful in the future.

\smallskip
\textbf{Leaf increasing.} We call a potential function $f$, a leaf increasing function if for every tree $T$, $v$ in $V(T)$ and $u\not\in V(T)$ then $f(v,T) < f(u, T \cup \{v,u\})$.

\begin{example}
	The function $f(v,T) = |\Asg(v,T)|$ is a leaf increasing potential function.
\end{example}

\smallskip
\textbf{Monotonic.} Given a potential function $f$, we say that $f$ is monotonic if for every tree $T$, nodes $v,u$ in $V(T)$ and tree $T'$ such that $V(T)\cap V(T') = \{u\}$, then $f(v,T)\leq f(v, T\cup T')$.

\begin{example}
	The function $f(v,T) = \#Leaves(T)$ is a monotonic potential function but it is not leaf increasing.
\end{example}

Before going deeper in the power of potential functions, we will introduce a very important property on how we expect roots to compare between different trees.

\begin{definition}[Regularity property]
	We say that a ranking $\preceq$ with the rooting-tree property enjoys the \emph{regularity property} if for every tree $T$, nodes $u,v$ in $V(T)$ such that $u\in \roots(T)$ and node $w$ not in $V(T)$, then $\roots(T+\{v,w\}) \subseteq \pi_{uv}\cup\roots(T)$.
\end{definition}

In the rest of this section we characterize the rankings capable of rooting trees by using potential functions. First, we show the following lemma which will be useful lately.

\begin{lemma}\label{lemma:functionAlg}
	Let $\preceq$ be a ranking  with potential function $f$ which is monotonic and leaf increasing. Let $T$ be any tree and $u,v$ in $V(T)$, where $\pi_{uv}:= u = w_1w_2...w_n=v$ is the unique path connecting $u$ to $v$ in $T$ and $|\pi_{uv}| > 2$.  Now, if $f(u, T-\{u,w_2\}) \leq f(v,T-\{v,w_{n-1}\})$ then $(u, T) \prec (w_2,T)$.
\end{lemma}
\begin{proof}
	In first place, since $f$ is a potential function for $\preceq$ we know that 
\begin{equation}\label{eq:eq7}
	(u, T) \prec (w_2,T) \text{ if and only if } f(u, T - \{u,w_2\}) < f(w_2,T - \{u,w_2\}).
\end{equation}

In consequence, we just have to prove the second inequality in equation~\ref{eq:eq7}. Now, because $f$ is monotonic we know that 
\begin{equation}\label{eq:eq8}
	f(w_2, T - \{u,w_2\}) \geq f(w_2, T-\{\{w_2, z\}\mid z\in (N(w_2)\backslash \{w_3\})\}). 
\end{equation}


Notice that $w_2$ in the tree $T-\{\{w_2, z\}\mid z\in (N(w_2)\backslash \{w_3\})\}$ is a leaf hanging from $w_3$. Therefore, by the leaf increasing property we know that 
\begin{equation}\label{eq:eq9}
	f(w_2, T-\{\{w_2, z\}\mid z\in (N(w_2)\backslash \{w_3\})\}) > f(w_3, T -\{w_3, w_2\}).
\end{equation}
Now, combining equation~\ref{eq:eq8} and \ref{eq:eq9} we have that 
\begin{equation}
	f(w_2, T - \{u,w_2\}) > (w_3, T -\{w_3, w_2\}).
\end{equation}

We can repeat this process until we reach $w_{n}$ and then 

\begin{equation}\label{eq:eq10}
	f(w_2, T - \{u,w_2\}) > (w_{n}, T-\{w_{n-1},v\}).
\end{equation}

Finally, by hypothesis we know that  $f(v, T-\{w_{n-1},v\}) \geq f(u, T-\{u,w_2\})$. Thus, this fact plus equation~\ref{eq:eq10} implies that

\begin{equation}
	f(w_2, T - \{u,w_2\}) > f(u, T-\{u,w_2\}).
\end{equation}

\end{proof}
Notices that lemma~\ref{lemma:functionAlg} applies when $|\pi_{uv}| = 2$ with the exception that $(u, T)\preceq (w_2, T)$ because in equation~\ref{eq:eq9} we can not apply the leaf increasing property. We will also need to state the fact that a leaf can never be a root under certain circumstances.

\begin{lemma}\label{lemma:Leavesnotroots}
	If $\preceq$ is a close under isomorphism ranking with leaf increasing and monotonic potential function $f$ then for every tree $T$ with $|V(T)| > 2$, if $w\in Leaves(T)$ then $w\not\in \roots(T)$.
\end{lemma}
\begin{proof}
Assume by contradiction there exists a tree $T$ and a leaf $h$ in $V(T)$ such that $\{h\}\subseteq \roots(T)$. Therefore, by the definition of $f$ we know that if $w$ is the parent of $h$, then $f(w, T-\{w,h\}) \leq f(h, (\{h\}, \emptyset))$. Now, if $w$ is a leaf in $T-\{w,h\}$ we know by leaf increasing that $f(w, T-\{w,h\}) > f(z, T-\{w,z\}-\{w,h\} )$ where $z$ is the parent of $w$ in $T-\{w,h\}$. If $w$ is not a leaf in $T-\{w,h\}$, we can prune $T-\{w,h\}$ until $w$ becomes a leaf in the pruned tree $T'$ and by monotonicity of $f$ we have that $f(w,T-\{w,h\})\geq f(w, T')$. Since $|V(T)|>2$ we know $|T'|>1$. Now, we can apply the leaf increasing property of $f$ over $T'$ and get that $f(w,T-\{w,h\}) > f(u, T')$ where $u$ is the parent of $w$ in $T'$. We can repeat this process until we reach a tree with just $1$ node $x$. Therefore, we will get that $f(h,(\{h\}, \emptyset)) > f(x, (\{x\}, \emptyset))$. Finally, we can use this fact to show that $(h, (\{h,x\}, \{\{h,x\}\})) \succ (x,  (\{h,x\}, \{\{h,x\}\}))$ which contradicts the fact that $\preceq$ is close under isomorphism.
\end{proof}

The following lemma exploits the close under isomorphism property of a ranking $\preceq$ to show that a potential function $f$ with respect to $\preceq$ is also close under isomorphism for certain trees. 
\begin{lemma}\label{lemma:isofunction}
	If $\preceq$ is a close under isomorphism rooting tree ranking with potential function $f$ then for every isomorphic pair $(v_1, T_1)\cong (v_2, T_2)$ such that $V(T_1)\cap V(T_2) = \emptyset$ then $f(v_1, T_1) = f(v_2, T_2)$.
\end{lemma}
\begin{proof}
	Since $\preceq$ is a rooting tree ranking, then $v_1$ and $v_2$ are the only isomorphic nodes that are connected in the tree $T_1\cup T_2+ \{v_1,v_2\}$. Therefore, it must be the case that $\roots(T_1\cup T_2+ \{v_1,v_2\}) = \{v_1,v_2\}$. This means that $(v_1, T_1) \equiv (v_2, T_2)$. Now, by definition of the potential functon $f$, we have that $f(v_1, T_1) \leq f(v_2, T_2)$ and $f(v_2, T_2)\leq f(v_1,T_1)$ concluding the proof.
\end{proof}

Now is time to characterize which rankings are able to root trees using potential functions.

\begin{theorem}\label{th:Charpotential}
	Let $\preceq$ be a close under isomorphism ranking with potential function $f$. Then, the following are equivalent
	
	\begin{enumerate}
		\item $\preceq$ enjoys the rooting tree property and regularity.
		
		\item $f$ is a monotonic and leaf increasing potential function.
	\end{enumerate}
\end{theorem}

\begin{proof}
	$2) \to 1)$. In first place, we will prove that $\preceq$ enjoys the AMOP property. 
	Fix an arbitrary tree $T$, node $v$ and let $u,w$ be two arbitrary neighbours of $v$ in $T$.
	By removing edges $\{u,v\}$ and $\{v,w\}$ we get a decomposition of $T$ into trees, $T_u, T_v, T_w$ containing $u,v,w$, respectively, such that
	\[ T = (T_v \cup T_u \cup T_w)+ \{u,v\} + \{v,w\}. \]
	Without loss of generality assume $f(w,T_w) \leq f(u,T_u)$.
	From leaf increasing we have $f(u,T_u) < f(v, T_u + \{u,v\})$ and using the monotonic property of $f$ we get $f(u,T_u) < f(v, (T_u + \{u,v\}) \cup T_v)$.
	Based on our assumption $f(w,T_w) \leq f(u,T_u)$, we conclude  $f(w,T_w) < f(v, (T_u + \{u,v\}) \cup T_v)$.
	This, combined with the potential function definition, implies that $(w,T) \prec (v,T)$.
	Hence, we just proved that out of every two neighbours at least one has smaller centrality than $v$ which implies the thesis. By claim~\ref{claim:AMOProot} we know that $\preceq$ enjoys the rooting tree property except for regularity.
	
	\smallskip
	In second place, we must prove that $\preceq$ satisfies the regularity property. For this we will use the counter positive of lemma~\ref{lemma:functionAlg}. This is, for any tree $T$ and nodes $u,v$ in $V(T)$ connected by a path $\pi_{uv}:=u = w_1w_2...w_n=v$ with $|\pi_{uv}|>2$, if $(w_2, T)\preceq (u,T)$ then $f(v, T- \{v,w_{n-1}\}) < f(u, T-\{u,w_2\})$. Suppose now by contradiction that $\preceq$ does not satisfy the regularity property. In other words, there exists a tree $T$, nodes $u,v $ in $V(T)$ and $w$ not in $V(T)$ such that $u\in \roots(T)$. Now, if $\pi_{uv} = z_1z_2...z_n$ is the path connecting $u$ and $v$ in $T$, then $\roots(T + \{v,w\}) \not\subseteq \pi_{uv}\cup\roots(T)$. In other words, there exists $x$ not in $\pi_{uv}\cup\roots(T)$ such that $x\in\roots(T+\{v,w\})$. We know that $x\not=w$ for lemma~\ref{lemma:Leavesnotroots}. Therefore, in one case, there exists $z_i\in \pi_{uv}$ (the closest to $x$) such that for every $j\not=i$ then $z_j\not\in \pi_{xz_i}$ and $|\pi_{xz_i}| > 2$. Set the path connecting $x$ to $z_i$ as $\pi_{xz_i} = y_1y_2...y_k$. Notice that $\pi_{xu} = y_1y_2...z_iz_{i-1}...z_1$. Therefore, since $x$ is in $\roots(T+\{v,w\})$, then $(x,T+\{v,w\}) \succeq (y_2, T+\{v,w\})$. Thus, by counter positive of lemma~\ref{lemma:functionAlg} we know that $f(x, T-\{x, y_2\}) > f(z_i, T-\{z_i, y_{k-1}\} + \{v, w\})$. We also know by the monotonic property of $f$ that $f(z_i, T-\{z_i, y_{k-1}\} + \{v, w\}) \geq f(z_i, T-\{z_i, y_{k-1}\})$. This implies that $f(x, T-\{x, y_2\}) > f(z_i, T-\{z_i, y_{k-1}\})$ and applying lemma~\ref{lemma:functionAlg} again we have that $(x, T) \succ (z_i, T)$ which is a contradiction with the fact that $(u, T) \succeq (z_i, T) \succeq (x, T)$ from claim~\ref{claim:AMOProot}. In the case that there is not a $z_i$ such that $|\pi_{xz_i}|> 2$ then $x$ must be connected to $u$. From this we can conclude in the same way that since $(x, T+\{v,w\}) \succeq (u,T+\{v,w\})$ then $f(x, T-\{x,u\}) \geq f(u, T+\{v,w\} - \{x,u\}) \geq f(u, T-\{x,u\})$  by monotonicity of $f$. Finally, since $u\in \roots(T)$ then $(u, T)\succeq (x, T)$ which means that $f(u, T-\{x,u\}) \geq f(x, T-\{x,u\})$ concluding that $f(u, T-\{x,u\}) = f(x, T-\{x,u\})$ and therefore $x\in \roots(T)$ which contradicts the fact that $x\not\in\pi_{uv}\cup\roots(T)$.
		
	\smallskip
	$1)\to 2)$. In first place, we will prove that $f$ satisfies the leaf increasing property. Take any tree $T$ and node $u$ in $T(V)$. If $w$ is a node not in $V(T)$ then $w$ is a leaf in $T\cup\{u,w\}$. Now, by close under isomorphism there exists a tree $T'\cong T$ such that $V(T+\{w,u\})\cap V(T') = \emptyset$. Therefore, for every node $z\in V(T)$ there exists an isomorphic node $z'\in V(T')$ such that $(z, T\cup T'+\{w,u\}) \cong (z', T\cup T'+\{w,u\})$. The only node that does not have an isomorphic node in $T\cup T'+\{w,u\}$ is $u$. In consequence, if $\{u\} \not= \roots(T\cup T'+\{w,u\})$ then $\roots(T\cup T'+\{w,u\})\not\subseteq E(T\cup T'+\{w,u\})$ which contradicts the fact that $\preceq$ satisfies the rooting property. Then, $u$ must be the only root in $T\cup T'+\{w,u\}$. Therefore, if $u'$ is isomorphic to $u$ in $T\cup T'+\{w,u\}$, then $(u', T\cup T'+\{w,u\}) \prec (w, T\cup T'+\{w,u\})$ which implies by the definition of a potential function and lemma~\ref{lemma:isofunction} that $f(u, T) = f(u', T') < f(w, T + \{w, u\})$.
	
	In order to prove that $f$ is monotonic, we will exploit isomorphism again. Take any pair of isomorphic trees $T$ and $T'$ such that $V(T)\cap V(T') = \emptyset$. Set nodes $u$ in $V(T)$ and $u'$ in $V(T')$ such that $(u, T)\cong (u', T')$. Let $w$ be a node in $V(T)$ and $H$ be a tree such that $V(T)\cap V(H) = \{w\}$. We know that $\roots(T\cup T' + \{u,u'\}) = \{u,u'\}$ because if any other node is a root, then we have isomorphic nodes with the higher ranking that are not connected in $T\cup T' + \{u,u'\}$. Now, by the regularity property of $\preceq$ we know that $(u', T\cup T' + \{u,u'\} \cup H) \preceq (u, T\cup T' + \{u,u'\} \cup H)$. In other words,  $\roots(T\cup T' + \{u,u'\} \cup H)$ might be a subset of $T\cup H$ by applying several times the regularity property. Finally, by definition of $f$, we have that $f(u, T\cup H)\geq f(u', T') = f(u, T)$ i.e $f$ is monotonic.
\end{proof}

Some direct applications of theorem~\ref{th:Charpotential} imply which centrality measures are able to root trees with regularity. 

\begin{corollary}
	$\textsc{Closeness}$ can root trees with regularity.
\end{corollary}

\begin{proof}
	We will prove that $\preceq_{\textsc{Closeness}}$ has potential function $f(v,T) = |V(T)|$ which is monotonic and leaf increasing. Fix $T$ as any tree with nodes $u,v$ such that $\{u,v\}\in E(T)$. Define $T_v$ as the portion of $T-\{u,v\}$ hanging from $v$ and $T_u$ the portion hanging form $u$ as well. We know that \begin{equation}\label{eq:close1}
		\sum_{x\in T}d_{T}(v,x) = \sum_{x\in T_v}d_{T_v}(v,x) + \sum_{x\in T_u} 1 + d_{T_u}(u,x) = \sum_{x\in T_v}d_{T_v}(v,x) + \sum_{x\in T_u}d_{T_u}(u,x) + |V(T_u)|
	\end{equation}. On the other hand, for $u$ we have that \begin{equation}\label{eq:close2}
\sum_{x\in T}d_{T}(u,x) = \sum_{x\in T_u}d_{T_u}(u,x) + \sum_{x\in T_v} 1 + d_{T_v}(v,x) = \sum_{x\in T_u}d_{T_u}(u,x) + \sum_{x\in T_v}d_{T_v}(v,x) + |V(T_v)|.
\end{equation} We now that, $\textsc{Closeness}(v, T) \leq \textsc{Closeness}(u, T)$ if and only if $\sum_{x\in T}d_{T}(v,x) \geq \sum_{x\in T}d_{T}(u,x)$. Thus, by equations~\ref{eq:close1} and \ref{eq:close2} we know that $\displaystyle\sum_{x\in T}d_{T}(v,x) \geq \displaystyle\sum_{x\in T}d_{T}(u,x)$ if and only if $|V(T_u)| \geq |V(T_v)|$. I.e $f(v,T) = |T|$ is a potential function for $\preceq_{\textsc{Closeness}}$. Now, clearly when we add a leaf $w$ connected to $u$ in a tree $T$ then $f(w, T+\{u,w\}) = |V(T)|+1 > |V(T)| = f(u, T)$. Therefore, $f$ is a leaf increasing function. On the other hand, if we $T$ is a tree, $u$ and $v$ two nodes in $V(T)$ and $T'$ is a tree such that $V(T)\cap V(T') = \{u\}$, then $f(v, T) = |V(T)| \leq f(v, T\cup T') = |V(T)|+|V(T')| - 1$. In other words, $f$ is also monotonic.

\end{proof}

\begin{corollary}
	$\textsc{Eccentricity}$ can root trees with regularity.
\end{corollary}
\begin{proof}
	The function $f(v,T) = \max_{u\in V(T)}d_{T}(v, u)$ is a potential function for $\preceq_{\textsc{ECC}}$ which is monotonic and leaf increasing.
\end{proof}

\begin{corollary}
	$\textsc{All-subgrahs}$ can root trees with regularity.
\end{corollary}
\begin{proof}
	The function $f(v,T) = |\Asg(v,T)|$ is a potential function for $\preceq_{\textsc{ASG}}$ which is monotonic and leaf increasing.
\end{proof}


==> app-openproblems.tex <==
\begin{enumerate}
\item Is it possible to exist 3 or more top nodes in a tree?

\item Is there a strategy to find the most central node even for trees?
\item Is it enough to axiomatize for leaves?
\item How to axiomatize ranking instead of centrality? What is the distribution of ranking in the graph?
\item Is it possible to add edges maintaining the most central node?
\item Are the most central nodes always isomorphs between them?

\item Are functions $H$ and $F$ necessary or are they implied by close under isomorphism?
\item What is the relation between the axioms and centroid, median or center of a tree?
\item Is it necessary an axiom to maximize centrality?
	\end{enumerate}
	

==> app-properties.tex <==
In this section we will look for properties that all subgraphs centrality satisfy in order to characterize this measure. Some properties are related with the value of centrality and others refer to the ranking between nodes defined by the measure.

\section*{Maximality for trees}

It is interesting to find some of this properties over simpler graphs like trees. Thanks to the cut vertex additivity, the computation of all subgraphs centrality in trees is easier (can be done in polynomial time). Therefore, it is natural to exploit this fact and try to find other measures satisfying similar characteristics. In first place, we introduce some definitions that will be useful further on.

\begin{definition}
	 Let $v$ be a cut vertex of a graph $G$ and $G_1,...,G_n$ all the subgraphs that partition $G$ and whose pairwise intersection is v, that is,  $V(G) = \bigcup_{i=1}^{n} V(G_i)$, $E(G) = \bigcup_{i=1}^{n} E(G_i)$ and $V(G_i)\cap V(G_j) =\{v\}$ for $i\not=j$.  Then a centrality measure $C$ has the cut vertex multiplicity property if $$C(v,G) = \prod_{i  = 1}^{n}C(v,G_i).$$
\end{definition}

If we reduce our centrality measure to just count subgraphs, i.e $C(v,G) = \Subg(v,G)$, this definition will satisfy cut vertex multiplicity. There is no consensus on if counting subgraphs is a better centrality measure than ASG because both has useful properties for different circumstances. Moreover, it could not even matter since both measures define the same ranking between nodes. Now we introduce a second property satisfied by counting subgraphs.

\begin{definition}
	Given a centrality measure $C$, a graph $G =(V,E)$ and a node $v\notin V(G)$. We say that $C$ satisfies the leaf addition property if $$C(v, G + \{u,v\}) = 1 + C(u,G)$$
	for any $u\in V(G)$. 
\end{definition}
In other words, any leaf from a graph will have a centrality closely related to its parent centrality without that child. This is not telling us how much the parent's centrality should change when adding a leaf.

\begin{theorem}
	\label{Theo:11}
	Given a tree $T=(V,E)$ and a node $v\in V(T)$. There exists at most one $u\in N(v)$ such that $\Acen(v,T)\leq \Acen(u,T)$.
\end{theorem}

\begin{proof}
	In first place, for a node $v\in V(T)$, we can enumerate the set $N(v) = \{u_1,u_2,...,u_n\}$. Therefore, we will define $t_k$ as the tree that is connected to $v$ by $u_k$. Now, by contradiction assume that exists $i\not=j$ such that $\Acen(v,T)\leq \Acen(u_i,T)$ and $\Acen(v,T)\leq \Acen(u_j,T)$. Because logarithm is a strictly increasing function, this is equivalent to say that $\Subg(v,T) \leq \Subg(u_i, T)$ and $\Subg(v,T) \leq \Subg(u_j, T)$. To simplify our notation we will define $N_k = \Subg(u_k, t_k)$. Therefore, by the vertex cut multiplicity and leaf addition, we have that $$\Subg(v,T) = \prod_{k = 1}^{n}\left(1+N_k\right) = (1+N_j)\prod_{k\not=j}\left(1+ N_k\right)= \prod_{k\not=j}\left(1+ N_k\right) + N_j\prod_{k\not= j}\left(1+N_k\right).$$ 
	
	On the other hand we have $$\Subg(u_j, T) = N_j\left(1+\Subg(v, T/t_j)\right) = N_j\left(1+\prod_{k\not=j}\left(1 + N_k\right)\right) = N_j + N_j\prod_{k\not=j}(1+N_k).$$
	
	By hypothesis we know that $$\Subg(u_j, T) - \Subg(v, T) = N_j - \prod_{k\not=j}\left(1 + N_k\right)\geq 0 \implies N_j - (1+N_i)\prod_{k\not\in \{i,j\}}(1+N_k) \geq 0$$ $$\implies \displaystyle\frac{N_j}{\prod_{k\not\in \{i,j\}}(1+N_k)} - 1 - N_i \geq 0 \implies \displaystyle\frac{N_j}{\prod_{k\not\in \{i,j\}}(1+N_k)} - 1 \geq N_i.$$
	
	We can use the same process to conclude that $$\displaystyle\frac{N_i}{\prod_{k\not\in \{i,j\}}(1+N_k)} - 1 \geq N_j.$$
	
	Arranging terms we get that $$\displaystyle\frac{N_j}{\prod_{k\not\in \{i,j\}}(1+N_k)} - 1 \geq N_i \geq \prod_{k\not\in \{i,j\}}(1+N_k) + N_j\prod_{k\not\in \{i,j\}}(1+N_k).$$
	
	Which clearly is a contradiction since $\displaystyle\frac{N_j}{\prod_{k\not\in \{i,j\}}(1+N_k)} - 1< \prod_{k\not\in \{i,j\}}(1+N_k) + N_j\prod_{k\not\in \{i,j\}}(1+N_k).$ 
\end{proof}

With this theorem we can conclude that in a tree the centrality goes from the most central node to the leaves, i.e there are not any discontinuity in the centrality distribution of a tree.


\begin{corollary}
	\label{cor:corollary11}
	Let $T=(V,E)$ be a tree, $v$ the most central node in $T$ and $u\in V(T)$ such that $u\not = v$. If $\pi:=v = w_1...w_n=u$ is the unique path connecting $v$ to $u$, then for every $i\in\{1,..,n\}, \Acen(w_i, T) \geq \Acen(w_{
	i+1}, T).$
\end{corollary}

\begin{proof}
	In first place it is clear that $\Acen(w_1, T) \geq \Acen(w_{
		2}, T)$ since $v$ is the most central node. Then, by induction for $i \geq 1$ you can conclude that $\Acen(w_{i+1}, T) \geq \Acen(w_{i+2}, T)$ because $\Acen(w_{i}, T) \geq \Acen(w_{
		i+1}, T)$ and $w_{i+1}$ can not have two neighbours with more centrality than him.
	
\end{proof}

Finally, it is interesting to know if there is possible to have $3$ most central nodes in a tree. This can not be the case because it would violate theorem~\ref{Theo:11}, but first we need the following lemma.

\begin{lemma}
	\label{Lemma:lemma11}
	Let $T=(V,E)$ be a tree and $v,u\in V(T)$ such that $u\not= v$ and both are most central nodes. Then $\{u,v\}\in E(T)$.
\end{lemma}

\begin{proof}
	Suppose that $\{u,v\}\notin E(T)$, then there must be a path $\pi:=u = w_1...w_n=v$ connecting $u$ and $v$ such that $n>2$. Since $u$ and $v$ have the same centrality, by corollary~\ref{cor:corollary1} we know that $\Acen(v,T)=\Acen(w_2,T) = ... = \Acen(u,T)$. This contradicts theorem~\ref{Theo:11} because $w_i$ for $i\in\{2,...,n-1\}$ have at least two neighbours with more or equal centrality than him.
\end{proof}
To conclude this section, we present two corollaries that answer our previous question and will be useful in further sections.
\begin{corollary}
	For every tree $T=(V,G)$, there exists at most 2 most central nodes. 
\end{corollary}

\begin{proof}
	By contradiction assume there are 3 most central nodes $u,v$ and $w$. Then, by lemma~\ref{Lemma:lemma11} the edges $\{u,v\}, \{v,w\}$ and $\{w,u\}$ are in $E(T)$. Therefore, we have a cycle in the tree. 
\end{proof}

\begin{corollary}
	\label{Col:Col22}
 Let $T=(V,E)$ be a tree and $u,v$ two nodes in $V(T)$ such that $\{u,v\}\in E(T)$ and $\Acen(v,T) = \Acen(u,T)$. Then $u$ and $v$ are the most central nodes.
\end{corollary}

\begin{proof}
	By contradiction suppose exists $x\in V(T)$ such that $x\not=v$ and $x\not=u$ that is the most central node. Without lose of generality define the path $\pi:=x=w_1...w_n=u$ such that for all $i, v\not= w_i$. By corollary~\ref{cor:corollary11} we know that for every $i, \Acen(w_i,T) \geq \Acen(w_{i+1})$. Therefore, $u$ has two neighbours $(w_{n-1}$ and $v$ ) with centrality greater or equal to him, which contradicts theorem~\ref{Theo:11}.
\end{proof}

Something remarkable about this result is that any centrality measure that satisfy cut vertex multiplicity and leaf addition will satisfy theorem~\ref{Theo:11} and therefore every previous result. Before ending this section we would like to show that having cut vertex additivity and leaf addition properties at the same time will derive in a non informative centrality measure  as stated in the next theorem.

\begin{theorem}\label{th:theo22}
	Given a tree $T=(V,E)$ and a centrality measure $C$ that satisfy leaf addition, cut vertex additivity and isolated vertex. Then $$C(v,T) = |E|$$ for every node v in $V(T)$.
\end{theorem}

\section*{Isomorphism and maximality}

In this section we will solve the problem of maximality and isomorphism. In particular, are most central nodes always isomorphs between them? We will create two counter examples for this question. The first one use two exponentially different graphs and for the second we will use a polynomial construction with trees.
\\
Given a tree $T=(V,E)$ and an arbitrary node $v$ in $V(T)$, define $n = \Subg(v,T)$.
 We know that the extreme of a line with $n$ nodes, $L_n$,  has $n$ connected subgraphs. Therefore, the extreme of the line $L_{n}$ has the same amount of subgraphs that $v$ in $T$. If $u$ is the extreme of $L_{n}$, define the tree $T' = T + L_{n} + \{u,v\}$. By ranking monotonicity axiom we know that $\Acen(v, G) = \Acen(u, G)$ and by corollary~\ref{Col:Col22} we conclude that $u$ and $v$ must be the most central nodes in $T'$. Clearly this construction use a line with an exponential amount of nodes in the centrality we want to generate our counter example. There is a smarter way to do this by a construction like the one in algorithm~\ref{Alg:alg1}.
 
 \begin{algorithm}[]
 	\SetAlgoLined
 	\KwIn{$k>0$ binary digits $(n)_2=d_1\ldots d_k$ such that $d_1=1$ }
 	\KwOut{$(T,u)$, with a tree $T=(V,E)$ and $u\in V$ such that $\Subg(T,u)=n$}
 	%initialization\;
 	
 	\SetKwFunction{BuildTree}{BuildTree}
 	\SetKwProg{Fn}{Function}{:}{}
 	\Fn{\BuildTree{$d_1\ldots d_k$}}{
 		$u:= v_{k-1}$\;
 		$v:= v_k$\;
 		\If{$k=1$}{
 			\KwRet $((\{u\},\emptyset),u)$\;
 		}
 		\If{$d_k=1$}{
 			$(V,E)\leftarrow$\BuildTree{$d_1\ldots d_{k-1}0$}\;
 			\KwRet $((V\cup\{v\},E\cup\{\{u,v\}\}),v)$\;
 		}
 		\If{$d_k=0$}{
 			$(V,E)\leftarrow$\BuildTree{$d_1\ldots d_{k-1}$}\;
 			\KwRet $((V\cup\{v\},E\cup\{\{u,v\}\}),u)$\;
 		}
 	}
 	
 	\caption{Tree construction with known $\Subg(T,u)$ (Sebastián Guerra).}
 	\label{Alg:alg1}
 \end{algorithm}
 \bigskip
 
This give us a polynomial size tree in the centrality we want. Therefore, we can connect the output of this algorithm to an arbitrary tree and generate a graph where the most central nodes are not isomorph between them.

\subsection*{At-most-one-parent imples rooting-trees}

The relevance of homogenous axiom relies on the implication about rooting trees. Using this axiom we can conclude that in a tree, the centrality goes from the most central node to the leaves. In other words, there are not any discontinuity in the centrality distribution of a tree.

\begin{corollary}
	\label{cor:corollary1}
	Let $C$ be an homogenous centrality measure, $T=(V,E)$ a tree graph, $v$ the most central node in $T$ according to $C$ and $u\in V(T)$ such that $u\not = v$. If $\pi:=v = w_1...w_n=u$ is the unique path connecting $v$ to $u$, then for every $i\in\{1,..,n\}, C(w_i, T) \geq C(w_{
		i+1}, T).$
\end{corollary}

\begin{proof}
	In first place it is clear that $C(w_1, T) \geq C(w_{2}, T)$ since $v$ is the most central node. Then, by induction for $i \geq 1$ you can conclude that $C(w_{i+1}, T) \geq C(w_{i+2}, T)$ because $C(w_{i}, T) \geq C(w_{i+1}, T)$ and $w_{i+1}$ can not have two neighbours with more centrality than him.
	
\end{proof}

Finally, it is necessary to prove if that there is not possible to have $3$ most central nodes in a tree. This can not be the case because it would violate the homogenous axiom, but first we need the following lemma.

\begin{lemma}
	\label{Lemma:lemma1}
	Let $C$ be an homogenous centrality measure, $T=(V,E)$ be a tree and $v,u\in V(T)$ such that $u\not= v$ such that both are most central nodes according to $C$. Then $\{u,v\}\in E(T)$.
\end{lemma}

\begin{proof}
	Suppose that $\{u,v\}\notin E(T)$, then there must be a path $\pi:=u = w_1...w_n=v$ connecting $u$ and $v$ such that $n>2$. Since $u$ and $v$ have the same centrality, by corollary~\ref{cor:corollary1} we know that $C(v,T)=C(w_2,T) = ... = C(u,T)$. This contradicts homogeneity because $w_i$ for $i\in\{2,...,n-1\}$ have at least two neighbours with more or equal centrality than him.
\end{proof}
To conclude one of the main results, we present two corollaries that will be useful in further sections.

\begin{corollary}\label{cor:corollary2}
	If $C$ is an homogenous centrality measure, then for every tree $T=(V,G)$ there exists at most 2 most central nodes. 
\end{corollary}

\begin{proof}
	By contradiction assume there are 3 most central nodes $u,v$ and $w$. Then, by lemma~\ref{Lemma:lemma1} the edges $\{u,v\}, \{v,w\}$ and $\{w,u\}$ are in $E(T)$. Therefore, we have a cycle in the tree. 
\end{proof}

\begin{corollary}
	\label{Col:Col2}
	Let $C$ be an homogenous centrality measure, $T=(V,E)$ be a tree and $u,v$ two nodes in $V(T)$ such that $\{u,v\}\in E(T)$ and $C(v,T) = C(u,T)$. Then $u$ and $v$ are the most central nodes in $T$ according to $C$.
\end{corollary}

\begin{proof}
	By contradiction suppose exists $x\in V(T)$ such that $x\not=v$ and $x\not=u$ that is the most central node. Without lose of generality define the path $\pi:=x=w_1...w_n=u$ such that for all $i, v\not= w_i$. By corollary~\ref{cor:corollary1} we know that for every $i, \Acen(w_i,T) \geq \Acen(w_{i+1})$. Therefore, $u$ has two neighbours $(w_{n-1}$ and $v$ ) with centrality greater or equal to him, which contradicts homogeneity.
\end{proof}
The most remarkable about these results is that any homogenous centrality measure can root trees. We summarize that in the following theorem.

\begin{theorem}
	$EP_{=}(\mathcal{C}_H)\subseteq \mathcal{C}_T$.
\end{theorem}
\begin{proof}
	We just have to add lemma~\ref{Lemma:lemma1}, corollary~\ref{cor:corollary1} and corollary~\ref{cor:corollary2}.
\end{proof}

\subsection*{Computing roots}

\begin{algorithm}[]
	\SetAlgoLined
	\SetKwFor{While}{while}{}{end while}
	\KwIn{Rooted tree $T$ and values $C(v,T_v)$ from the root to the leaves.}
	\KwOut{Most central node of $T$.}
	%initialization\;
	
	\SetKwFunction{MC}{MostCentral}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\MC{$C, T$}}{
		$v= root(T)$\;
		
		\ForEach{$u\in V(G)$}{$u.color=white$\;}
		
		\While{$v.color==white$:}{
			$v.color=black$\;
			$A = \arg\max_{u\in N(v)}C(u,T-\{u,v\})$\;
			\If{$|A|>1$ \textsc{or} $C(A[0],T-\{A[0],v\})\leq C(v,T-\{A[0],v\})$\;}{\KwRet $v$\;}
			\Else{$v = A[0]$\;}
		}
		
		\KwRet $v \in U$\;
	}
	
	\caption{Computing the most central node from a rooted tree.}
	\label{Alg:alg3}
\end{algorithm}
\bigskip

Algorithm~\ref{Alg:alg3} correctness is a direct consequence of the following lemma.

\begin{lemma}\label{lemma:algorithmOsk}
	For every tree $T$ and node $v\in V(T)$, if there exists $w\not=u\in N(v)$ such that $C(w,T-\{w,v\})\geq C(u,T-\{u,v\})$ then $C(v,T)\geq C(u,T)$.
\end{lemma}

In other words, if a neighbour of $v$ has the greatest centrality in its subtree, then this is the only possible node with greatest centrality than $v$.

\subsection*{Functions for centrality measure}
%\subsubsection{Cut vertex function}
In order to make a difference between meaningful definitions of centrality, we need to stablish the way a  measure grows and behaves within trees. As we already know, allsubgraphs centrality and counting subgraphs satisfy the cut-vertex additivity and cut-vertex multiplicity properties respectively. While counting edges also satisfies cut-vertex additivity as seen in theorem~\ref{th:theo22}. More over, this property plus isolated constant and Leaf adition function completely characterize counting edges in trees. To generalize this ideas, we ask for a function that explain the way a centrality measure is added in a cut vertex.

\smallskip
\ax{6}{Cut-vertex Function} Given a centrality measure $C$, we say that $C$ satisfy the cut-vertex function axiom if there exists $F:\mathbb{R}\times\mathbb{R} \to\mathbb{R}$ such that if $T_1$ and $T_2$ are two disjoint trees where $V(T_1)\cap V(T_2) = \{v\}$, then $$C(v, T_1\cup T_2) = F(C(v,T_1), C(v,T_2)).$$
\smallskip


Directly from this definition we can conclude that $F$ must be commutative i.e $F(C(v,T_1), C(v,T_2)) = F(C(v,T_2), C(v,T_1))$  and associative i.e $F(F(C(v,T_1),C(v,T_2)), C(v,T_3)) = F(C(v,T_1),F(C(v,T_2), C(v,T_3)))$ since the centrality of $v$ is uniquely defined. For this reason from now on we will simplify our notation as $F(a,b,c) = F(F(a,b),c)= F(a,F(b,c))$.

All previous properties can not characterize the ranking defined by allsubgraphs or counting subgraphs since counting edges satisfy all of them. In fact, we need to ask for more restrictions to the function $F$.

\begin{definition}
	For a cut-vertex function $F$ we say that it is increasing if for every cut vertex $v$, then $C(v,T_1) \leq F(C(v,T_1),C(v,T_2))$ and $C(v,T_1) = F(C(v,T_1),C(v,T_2))$ iff $T_2$ is an isolated vertex.	
\end{definition}
In other words we want that this function $F$ increase whenever we compute the centrality of a cut vertex of two disjoint trees that are not isolated vertices. Therefore, we can translate the increasing property as 
\begin{equation}\label{eq:identity}
	\forall a, a = F(k,a) = F(a,k)
\end{equation}
\begin{equation}
	\forall a\forall b, (a\not=k \wedge b\not= k) \implies (a< F(a,b)\wedge b < F(a,b))
\end{equation}

Finally, equation~\ref{eq:identity} means that $k$ is an identity for $F(\cdot,\cdot)$. Combining this with the commutative and associative properties it implies that $(k,F)$ forms a commutative monoid in $R^{\geq k}$. For this reason, from now on we denote 

\begin{eqnarray}
	a\ast b :=& F(a,b)\\
	\mathds{1} :=& k
\end{eqnarray}
where $(\mathbb{R}^{\geq k}, \ast, \mathds{1})$ is a commutative monoid and $a<a\ast b$ when $b>\mathds{1}$.

%\subsubsection{Leaf adition function}

Now it is necessary to stablish a function that tells us how centrality is transferred to a leaf from its parent. In other words, when a new leaf is added, we assume there is a value this leaf is receiving depending on its parent importance.

\smallskip
\ax{7}{Leaf addition function} Let $C$ be a centrality measure and $T$ a tree such that $u$ is not a node from $T$. We say that $C$ has the Leaf adition function property if there exists a function $H_C:\mathbb{R}^{+}\to \mathbb{R}^{+}$ such that $C(u, T + \{u,v\}) = H_C(C(v, T))$.
\smallskip

For example, in all subgraphs centrality when $u$ is not in $V(T)$ we have that $\Acen(v, T)= \log(\Subg(v,T))\implies k(\Acen(v,T)) = 2^{\Acen(v,T)} = \Subg(v,T)$. Therefore, for allsubgraphs centrality $\Acen(u, T+\{u,v\}) = \log(1+k(\Acen(v,T))) = H_{\Asg}(\Acen(v,T))$. On the other hand, for counting subgraphs we have $\Subg(u,T +\{u,v\}) = 1 + \Subg(v,T) = H_{\Subg}(\Subg(v,T))$. Finally, we can define the edges centrality as $C_{|E|}(v,G) = |E(G)|$. In this case, we have $C_{|E|}(u,T + \{u,v\}) = 1 + C_{|E|}(v,T) = H_{|E|}(C_{|E|}(v,T))$. Therefore, this proves that isolated constant, Leaf adition function and cut-vertex function are not very informative by themselves because very useless centralities as counting edges have the same function $H$ as another more complex as counting subgraphs. For this reason we want to ask for more restriction to the functions $H$ and $\ast$. In first place, $H$ must be a strictly increasing function since the centrality of a parent should be at least completely transferred to their son.

\begin{definition}
	If $C$ is a centrality measure satisfying Leaf adition function. We say that $H_C$ is strictly increasing if $C(v,T)< H_C(C(v,T)) = C(u,T + \{u,v\})$ for a node $u\not\in V(T)$.
\end{definition}

%\begin{definition}
%	If $C$ is a centrality measure satisfying Leaf adition function and cut-vertex function. We say that $H_C$ is bounded by $F_C$ if $H_C(C(u, T-v)) \leq H_C(k)\ast C(u, T-v)$ for a leaf $v$ hanging from $u$.
%\end{definition}

%In other words, if a centrality measure satisfies both definition. The importance of a leaf must be strictly greater than his parent importance before adding it to the tree. Simultaneously, the centrality of its parent should be greater than his after we add the leaf. 

This property can be translated as $\forall a, a < H_C(a)$. The intuition behind strictly increasing functions is based on how parents pass their centrality over descendants. It is natural to think that every child it least as important as their parents. However, we ask for strictly increasing because we want that centrality actually grow for more complex structures. 

On the other hand, to have a more interesting set of properties we want that $\ast$ respect the centrality asymmetry when connecting two disjoint components.

\smallskip
If a centrality measure preserve asymmetry it is equivalent to say that over $(\mathbb{R}^{\geq k},\mathds{1},\ast, H), 
$ $$\forall a,b, \text{ if } a\leq b \iff a\ast H(b)\leq b\ast H(a).$$
This particular property is where counting edges fails. When we connect two trees, every node in the new graph has the same centrality value and therefore, it does not preserve the asymmetry.

Finally, we want that $\ast$ preserve order. This is a much stronger property but has a lot of intuition in the context of trees.

\smallskip
Preserving order can be translated to $\forall a,b,c, a < b\iff a\ast c < b \ast c$ which means that $(\mathbb{R}^{\geq k}, \ast, \mathds{1}, \leq)$ is and ordered commutative monoid.



==> app-rankings.tex <==

A centrality measure $C$ naturally defines a ranking between the vertices of a graph $G$: the greater the score the more relevant a vertex is in $G$. In fact, a measure $C$ allows to compare the relevance of vertices between different graphs. Specifically, if we have pairs $(v_1, G_1)$ and $(v_2, G_2)$ one can say that $v_1$ in $G_1$ is less relevant or equal than $v_2$ in $G_2$ if, and only if, $C(v_1, G_1) \leq C(v_2, G_2)$. Note that we can compare different vertices depending their context, and this naturally defines what we call a \emph{centrality ranking}. As we will see, these ranking allows to leverage the properties of centrality measures to rankings, and study them in a more abstract sense.   

Recall that $\cN$ are all pairs $(v, G)$ such that $v \in V(G)$. A centrality ranking $\preceq$ over graphs (or just a ranking) is any \emph{total quasi-order} over $\cN$. Formally, $\preceq$ is a relation over $\cN$ that is reflexive, transitive, and connected (i.e., for every $(v_1, G_1)$ and $(v_2, G_2)$, either $(v_1, G_1)\preceq(v_2, G_2)$ or $(v_2,G_2)\preceq (v_1, G_1)$). We also say that $(v_1, T_1)$ is equivalent to $(v_2, T_2)$ if $(v_1, T_1) \preceq (v_2, T_2)$ and $(v_2,T_2) \preceq (v_1, T_1)$. We write this as $(v_1, T_1) \equiv (v_2, T_2)$ when $\preceq$ is clear from the context. 
Note that $\equiv$ defines an equivalence relation over $\cN$. Intuitively, we have that $(v_1, G_1) \preceq (v_2, G_2)$ when $v_1$ in $G_1$ is less relevant or equal than $v_2$ in $G_2$, and $(v_1, G_1) \equiv (v_2, G_2)$ when both are equally relevant. 
Finally, we write $(v_1, T_1) \prec (v_2, T_2)$ when $(v_1, T_1) \preceq (v_2, T_2)$ but $(v_1, T_1) \not \succeq (v_2, T_2)$, namely, when $v_1$ in $G_1$ is strictly less relevant than $v_2$ in $T_2$.

Centrality measures are a particular case of a centrality rankings in the sense that every measure $C$ defines a ranking $\preceq_C$, such that $(v_1,G_1) \preceq_C (v_2,G_2)$ if, and only if, $C(v_1,G_1) \leq C(v_2,G_2)$. Nonetheless, it is not directly clear how to deduce a centrality measure from an arbitrary ranking. For this reason we see rankings as an abstraction of a centrality measure, where only the order between vertices and graphs is important. From now on, we refer to the natural ranking defined by a centrality measure $C$ as $\preceq_C$.

It is worth noticing that given that a ranking $\preceq$ is total, then for any finite set $\{(v_i, G_i)\}_i$ we can define the minimum and maximum element with respect to $\preceq$ (i.e., up to the equivalence relation $\equiv$). Namely, $\max_\preceq\{(v_i, G_i)\}_i$ is well-defined and it is a set of all pairs $(v, G) \in \{(v_i, G_i)\}_i$ such that $(v_i, G_i) \preceq (v, G)$. Furthermore, for every other pair $(v', G') \in \max_\preceq\{(v_i, G_i)\}_i$ it holds that $(v, G) \equiv (v', G')$. For this reason, the most central nodes in a graph $G$ with respect to $\preceq$ is well-defined and it is $\max_\preceq \{(v, G) \mid v \in V(G)\}$. 




%In first place we will give an extended definition of a ranking given a centrality measure.
%
%\begin{definition}
%For a centrality measure $C$, we define the ranking $\extrank{C}$ as following. For every two pairs $(v_1, G_1)$ and $(v_2, G_2)$, then $(v_1, G_1)\extrank{C} (v_2, G_2)$ if and only if one the following holds
%
%\begin{enumerate}
%	\item $G_1 \cong G_2$ and $C(v_1, G_1) \leq C(v_2, G_2)$.
%	
%	\item $C(v_1, G_1 + G_2 + \{v_1, v_2\}) \leq C(v_2, G_1+ G_2+ \{v_1, v_2\})$.
%	
%\end{enumerate}
%\end{definition}
%It is not clear when the relation $\extrank{C}$ is a proper ranking. This is, for which measures $C$, $\extrank{C}$ is a total quasi order over $\cN$? 
%\begin{lemma}\label{lemma:bridge}
%	For two pairs $(v_1, T_1)$ and $(v_2, T_2)$, then $\textsc{Closeness}(v_1, T_1 + T_2 + \{v_1,v_2\})\leq \textsc{Closeness}(v_2, T_1 + T_2 + \{v_1, v_2\})$ if and only if $|V(T_1)| \leq |V(T_2)|$.
%\end{lemma}
%\begin{example}
%	The relation $\extrank{\textsc{Closeness}}$ is a ranking.
%\end{example}
%\begin{proof}
%	In first place, $\extrank{\textsc{Closeness}}$is reflexive since for every $(v_1, T_1)$ then $T_1\cong T_1$ and $C(v_1, T_1) = C(v_1, T_1)$. Therefore, $(v_1, T_1)\extrank{\textsc{Closeness}} (v_1, T_1)$. Now, to prove transitivity, we need lemma~\ref{lemma:bridge}. Fix pairs $(v_1, T_1)$, $(v_2, T_2)$ and $(v_3, T_3)$ such that $(v_1, T_1)\extrank{\textsc{Closeness}} (v_2, T_2)$ and $(v_2, T_2 ) \extrank{\textsc{Closeness}} (v_3, T_3)$. In first case, we have that $T_1 \cong T_2$ but $T_2 \not\cong T_3$. In this case we know that by lemma~\ref{lemma:bridge} we know that $|V(T_2)| \leq |V(T_3)|$. At the same time, since $T_1\cong T_2$ then $|V(T_1)| =|V(T_2)|$. Thus, $\textsc{Closeness}(v_1, T_1+ T_3 + \{v_1, v_3\}) \leq \textsc{Closeness}(v_3, T_1+T_3 +\{v_1, v_3\})$ which implies $(v_1, T_1)\extrank{\textsc{Closeness}}(v_3, T_3)$. In second place, it could be the case that $T_1\not\cong T_2$ but $T_2\cong T_3$. We can use a similar argument since $|V(T_1)| \leq |V(T_2)|$ by lemma~\ref{lemma:bridge} and $|V(T_2)| = |V(T_3)|$ by isomorphism. Therefore, $(v_1, T_1)\extrank{\textsc{Closeness}}(v_3, T_3)$. Finally, when $T_1\cong T_2\cong T_3$ we just have that $\textsc{Closeness}(v_1, T_1)\leq \textsc{Closeness}(v_2, T_2) \leq \textsc{Closeness}(v_3, T_3)$ which implies $\textsc{Closeness}(v_1, T_1)\leq \textsc{Closeness}(v_3, T_3)$ by transitivity of $\leq$.
%\end{proof}
%\jorge{The case that $T_1\cong T_3$ is missing!!!}
%
%Another way to extend the natural ranking defined by a centrality measure is by weighting a node importance by the amount of node in its graph. We define this extension as follow
%
%\begin{definition}
%	For a centrality measure $C$, we define the ranking $\extrankk{C}$ as, for every $(v_1, T_1)$ and $(v_2, T_2)$ then $(v_1, T_1)\extrankk{C}(v_2, T_2)$ if one of the following holds
%	
%	\begin{enumerate}
%		\item $|V(T_1)|< |V(T_2)|$.
%		\item $|V(T_1)| = |V(T_2)|$ but $C(v_1, T_1)\leq C(v_2, T_2)$.
%	\end{enumerate}
%	
%\end{definition}


==> intro.tex <==
Centrality measures are fundamental tools of network analysis. 
They are used in a plethora of applications from various areas, such as assessing the importance of websites by search engines~\cite{page1999pagerank}, finding people who are more likely to spread a disease in the event of an epidemic~\cite{Dezso:Barabasi:2002} or highlighting cancer genes in proteomic data~\cite{Ivan:Grolmusz:2010}. 
In all these applications, people use centrality measures to assess graph data and rank which nodes are the most relevant by only using the structure of the graph.

To date, except for the most popular degree, closeness and betweenness centralities, more than 200 measures have been proposed in the literature.
These measures assess the position of a vertex in the network based on various aspects which makes it hard to compare their properties.
Since dozens of new measures are proposed every year, it becomes more and more difficult to choose a measure for a specific application at hand. 
That is why, in recent years, efforts at understanding and explaining differences between existing measures have intensified.
This is also one of the main goals of this work.

Even in the case of tree structures, centrality measures vary significantly. 
Specifically, in the same tree, different measures indicate different vertices as the most central.
For example, consider a line graph: while the middle vertex (or vertices) are ranked first according to most centrality measures, PageRank, one of the most popular centrality measures, puts the second and the second-to-last vertices at the top of the ranking.
This shows that not only different measures select different vertices, but even one measure may select several vertices from different parts of the tree as the most~important.

This paper aims to understand how centrality measures operate on trees, as we believe this is a necessary step to explain their behavior on general graphs. Indeed, trees have always played a central role in representing structured data and, more generally, in finding efficient algorithms over families of graphs (e.g., families with bounded treewidth). Moreover, trees have a more amenable structure than general graphs, given that, among other properties, every edge is a cutting edge, and there is a unique path between any two nodes. For these reasons, we believe that studying how centrality measures behave over trees could give deep insights on understanding centrality measures over graphs.
 %Here, we want to follow a principle approach, where centralities measures are understood as a whole and not as isolated objects.  

Towards this goal, in this paper we attack the question of which centrality measures select one most central place in a network, namely, which defines a root for each tree. 
%For answering this question, we want to follow a principle approach, where centralities measures are understood as a whole and not as isolated objects.  
To this end, we introduce the \emph{rooting property} which states a measure selects one or two adjacent vertices in a tree as the most important, and the importance decreases from them in all directions. We found that closeness, eccentricity, and all-subgraphs centralities satisfy this rooting property but often rank different vertices at the top. We call the vertex (or two vertices) ranked first the ``root'' and say such measures \emph{root~trees}.

To understand what distinguishes measures that root trees we focus on the question: how to choose which out of two adjacent vertices is more central? 
We observe that most centrality measures, including all standard ones that root trees, answer this question by comparing subtrees of both vertices.
More precisely, we introduce a framework of \emph{potential functions} that assess the quality or ``potential'' of an arbitrary tree.
Now, we show that for most centrality measures, including degree, closeness, and betweenness, admit a potential function such that the vertex which subtree has higher potential value is considered more central.

Now, we show that if a centrality measure has a potential function, then it roots trees if, and only if, the potential function is \emph{symmetric}.
This property means that the potential of a tree is larger than the potential of any proper complete subtree. 
In particular, the potential function of closeness, eccentricity, and all-subgraphs centrality are symmetric, but the potential functions of degree and betweenness centralities are not; as a result, the later centralities do not root trees.

We use our framework of potential functions to understand better the class of measures that root trees. More specifically, we show three applications of potential functions. Our first application is to study efficient algorithms for computing a root when centrality measures have potential functions and root trees. A naive algorithm for this task takes quadratic time over a tree: by calculating the centrality measure for each vertex and then choosing the most central vertex. Instead, by exploiting symmetric potential functions, we show that, given a tree $T$, we can compute the most central vertex in time $\mathcal{O}(|T|\log(|T|))$ whenever one can calculate the potential function locally. Interestingly, this general algorithm works independently of the centrality measures and only depends on the potential function.

Our second application is to understand desirable properties over rooting tree measures. Although a centrality measure could root trees, it can behave inconsistently. For instance, a rooting centrality measure could choose the root of a tree $T$ close to a leaf when the size of $T$ is even and far from the leaves when the size of $T$ is odd. Therefore, we study when centrality measures consistently root trees through their potential functions. We propose a monotonicity property that imposes additional consistency conditions on how the root is selected and characterizes which potential functions satisfy this property. 

Our last application shows how to design and build new potential functions that consistently root trees. Specifically, we present infinitely many constructive potential functions that satisfy all properties discussed so far. In particular, the algorithm for finding the root applies to any of them. We believe that this family of measures is interesting in its own right and can be used in several data-driven scenarios to discover or learn how to choose the root of data trees.

%\clearpage
\paragraph{Related work}
Our work belongs to a broad literature that focuses on the analysis of theoretical properties of centrality measures.
The classic approach is to analyze standard centrality measures with respect to simple desirable properties.
Different sets of desirable axioms have been proposed over the years by \cite{sabidussi1966centrality}, \cite{Nieminen:1973}, \cite{boldivigna} and \cite{Boldi:etal:2017}.
Similarly, in our work, we propose several properties specific for trees and study which are satisfied by standard centrality measures.

Another approach is to create a common framework for large classes of centrality measures. 
In such frameworks, centrality measures are presented as a function of some underlying structure of a graph.
Hence, the emphasis is put more on the differences between these functions for various measures that the framework covers.
In this spirit, classes of measures based on nodal statistics~\cite{Bloch:etal:2019}, coalitional game theory~\cite{Skibski:etal:2018:gtc}, subgraphs~\cite{RiverosS20} and vitality functions~\cite{Skibski:2021:vitality} have been analyzed in the literature.
Our framework based on potential functions can be considered as an example of such approach, for the case of trees.

Yet another approach, less related to our work, is to focus on one or several similar measures and provide their full axiomatic characterization. 
In this spirit, axiomatizations of PageRank~\cite{Was:Skibski:2018:pagerank}, eigenvector \cite{Kitti:2016}, beta-measure and degree \cite{Brink:Gilles:2000} and many more have been developed in the literature.

There is also a line of research that studies methods for solely choosing one most central vertex in a tree that does not necessarily come from the centrality analysis (see, e.g., \cite{Reid:2011} for an overview).
However, such methods coincide with the top vertices selected by centrality measures that we consider in our work. In particular, the center of a tree coincides with eccentricity, and the median, as well as the centroid of a tree, coincides with closeness centrality.

\paragraph{Organization} We structure the paper as follows. Section~\ref{Sec:preliminaries} presents the main definitions used in the paper. In Section~\ref{Sec:rooting} we define the rooting property and discuss some of its consequences. Section~\ref{Sec:potential} introduces potential functions and the main characterization of the rooting property. Section~\ref{Sec:alg} presents an algorithm to find the root, and Section~\ref{Sec:regularity} discuss measures that consistently root trees. Section~\ref{Sec:alphabetagamma} is to show a family of potential functions that consistently root trees. Finally,  Section~\ref{Sec:concl} presents some concluding remarks.

==> intro_first_cycle.tex <==
Centrality measures are fundamental tools for network analysis. They are used in a plethora of applications from various areas of science, such as finding people who are more likely to spread a disease in the event of an epidemic~\cite{Dezso:Barabasi:2002} or highlighting cancer genes in proteomic data~\cite{Ivan:Grolmusz:2010}. In all these applications, people use centrality measures to assess graph data and rank which nodes are the most relevant by only using the graph's structure.

Databases have also incorporated centrality measures to rank objects in graph data. Probably the first use of a centrality measure in a data management problem is by Google search engine, which successfully introduced PageRank~\cite{page1999pagerank} for assessing the importance of a website on the web. From here, centrality measure has found its way in data management systems, for example, to rank nodes in graph databases (e.g., Neo4J~\cite{neo4j}) or in RDF data~\cite{zhang2007ontology}. 
Indeed, today any graph analysis tool contains a module for computing centrality measures which graph data scientists intensively use~\cite{newman2018networks}.

One could see centrality measures over graphs as an instance of a general database problem: find the most central data object in the data model given its underlying structure. The data model could be a relational database, an object-oriented database, an RDF database, or even a tree-structure database. For all these cases, the principle should be the same as for graphs: the more relevant the data object is for its data model, the more central it should be. In this paper, we refer to this problem as \emph{data centrality} where one would like to have (data) centrality measures that assess a database and rank their data objects by importance. 

Unfortunately, the database community has not formally studied the principles of data centrality yet. Apart from some applications over graph data like above, there is no research program on how we can measure the centrality of data objects and what their property should be. There is a lack of understanding even for the popular centrality measures over graphs. Indeed, this is why efforts at understanding and explaining differences between existing centrality measures over graphs have intensified in recent years~\cite{boldivigna,skibski2016attachment}.

With this paper, we want to initiate a research program on data centrality from the most simple data model: trees. Specifically, we would like to understand how centrality measures choose the most central nodes in trees: why some measures define a single important node (usually called the root) and why others do not. Centrality measures like closeness or eccentricity (see Section~\ref{Sec:preliminaries} for their definitions) always define one node or two adjacent nodes as the most central for every tree. Still, for other popular centrality measures like PageRank the set of the most central nodes is often large and consists of nodes far from each other. For instance, in a line graph, the middle node is intuitively the most central, but PageRank puts the second and the second-to-last vertices at the top of the ranking. Surprisingly, this simple question regarding ``tree rooting'' is not well understood yet, but one could say that it is \fix{fundamental to} any theory for data centrality. 
%\jorge{Why? I would stress the fact that this is expected when you just care about the structure.}

%Why should we care about centrality measures over trees? 
Although some databases use a tree data model, the most relevant problems regarding data centrality are for graph data or relational data. Nevertheless, we see several reasons for starting the study of data centrality on trees. First, arguably trees are the most simple and still non-trivial model to begin the study of data centrality. Indeed, trees have a more amenable structure than general graphs, given that, among other properties, every edge is a cutting edge, and there is a unique path between any two nodes. Second, every theory about data centrality should include trees, and it should answer similar questions like the one stated above. So, understanding centrality measures over trees could guide the study for other data models. Third and last, trees are probably the most ubiquitous data structure in computer science. Therefore, studying data centrality over trees could be helpful to other areas beyond databases. 

In this paper, we attack the question of which centrality measures \fix{always} select one most central place in a \fix{tree}, namely, which defines a root for each tree. For this, the main contributions are as follows:
\begin{enumerate}
	\item We introduce the \emph{tree rooting property} which states \fix{that} a measure selects one or two adjacent vertices in a tree as the most important, and the importance decreases from them in all directions. We found that closeness, eccentricity, and all-subgraphs centralities (see Section 2) satisfy this rooting property but often rank different vertices at the top. Instead, measures like degree and betweenness do not satisfy this property. We call the vertex (or two vertices) ranked first the ``root'' and say \fix{that} such measures \emph{root~trees}.
	
	\item To understand what distinguishes measures that root trees we focus on the question: how to choose which out of two adjacent vertices is more central? 
	We observe that most centrality measures, including all standard ones that root trees, answer this question by comparing subtrees of both vertices.
	More precisely, we introduce a framework of \emph{potential functions} that assess the quality or ``potential'' of an arbitrary tree.
	Now, we show \fix{that} most centrality measures admit a potential function such that the vertex which subtree has higher potential value is considered more central.
	
	\item We show that if a centrality measure has a potential function, then it roots trees if, and only if, the potential function is \emph{symmetric}.
	This property means that the potential of a tree is larger than the potential of any proper complete subtree. 
	In particular, the potential function of closeness, eccentricity, and all-subgraphs centrality are symmetric, but the potential functions of degree and betweenness centralities are not; as a result, the later centralities do not root trees.
	
	\item We use our framework of potential functions to understand better the class of measures that root trees. More specifically, we show three applications of potential functions. Our first application is to study efficient algorithms for computing a root when centrality measures have potential functions and root trees. A naive algorithm for this task takes quadratic time over a tree: by calculating the centrality measure for each vertex and then choosing the most central vertex. Instead, by exploiting symmetric potential functions, we show that, given a tree $T$, we can compute the most central vertex in time $\mathcal{O}(|T|\log(|T|))$ whenever one can calculate the potential function locally. Interestingly, this general algorithm works independently of the centrality measures and only depends on the potential function.
	
	\item Our second application of potential functions is to understand desirable properties over tree rooting measures. Although a centrality measure could root trees, it can behave inconsistently. For instance, a rooting centrality measure could choose the root of a tree $T$ close to a leaf when the size of $T$ is even and far from the leaves when the size of $T$ is odd. Therefore, we study when centrality measures consistently root trees through their potential functions. We propose a monotonicity property that imposes additional consistency conditions on how the root is selected and characterizes which potential functions satisfy this property. 
	
	\item Our last application shows how to design and build new potential functions that consistently root trees. Specifically, we present infinitely many constructive potential functions that satisfy all properties discussed so far. In particular, the algorithm for finding the root applies to any of them. We believe that this family of measures is interesting in its own right and can be used in several data-driven scenarios to discover how to choose the root of data trees.
\end{enumerate}
\paragraph{Organization} We structure the paper as follows.
We end this section by providing some related work. 
Section~\ref{Sec:preliminaries} presents the main definitions used in the paper. In Section~\ref{Sec:rooting} we define the tree rooting property and discuss some of its consequences. Section~\ref{Sec:potential} introduces potential functions and the main characterization of the tree rooting property. Section~\ref{Sec:alg} presents an algorithm to find the root, and Section~\ref{Sec:regularity} discuss measures that consistently root trees. Section~\ref{Sec:alphabetagamma} is to show a family of potential functions that consistently root trees. Finally,  Section~\ref{Sec:concl} presents some concluding remarks.

\paragraph{Related work}
\input{../Sections/related_work}

==> reviews.tex <==

\noindent
Dear reviewers,
\vspace*{0.4cm}

We wish to thank you for your thorough, insightful and constructive comments.
This paper is a revised manuscript of the version submitted to ICDT 2023 first cycle.
In the process of revising the paper, we have addressed your comments and suggestions.  
We have highlighted changes in \fix{blue}. Given the new material and space restrictions, we had to move the proof of Theorem~\ref{theo:rooting} to the appendix and remove the outline of the paper in the introduction. 
%OS: I think we cannot say that changes are major
%Please note that this resulted in major changes to the paper, which we have highlighted in \fix{red}.

The most important changes, which address the main revision items, are the following:

\paragraph{Motivation}
We agree that the motivation regarding ``data centrality'' was not correctly presented in the previous version. Although we believe this is an exciting research area for the community, our work does not have enough evidence to support this motivation. Moreover, the previous introduction did not support this correctly. For this reason, we have rewritten the introduction to better frame the work and explain the contributions. 
In particular, we better understand now that our principle approach tries to understand different centrality measures over graph families instead of previous research that studies classes of measures on all graphs. Thus, our work loses in generalizing the results to all graphs, but it gains insights into all measures. We change the motivation regarding this direction, and we hope that it aids in understanding the paper's contributions. Also we change the title of the paper accordingly.

\paragraph{Extensions and applications}
We added a new section to highlight the extensions and impact of our results. In this section, we present some preliminary ideas on how to apply potential functions to data management scenarios. Further, we show some connections of how one can generalize the notion of potential function to other graph classes.
\medskip

Below, we also provide a detailed list of answers and explanations to all the reviewer comments. %excluding those comments that we have already addressed above.

%Below we also provide a detailed list of answers and explanations to other reviewer comments, excluding those comments that we have already addressed above.
\vspace*{0.4cm}

%Note: We have copy and pasted the received reviewers’ comments and formatted them, while the corresponding answers are right below.
We sincerely hope that this new version of the manuscript sufficiently improves on the previous version, and that it will be considered for presenting in ICDT.

\vspace*{0.4cm}

\noindent
Best Regards,
\medskip

The authors.




\subsection{Response to Reviewer 1}

\begin{reviewer}
It is not clear in what way Definition 16 corresponds to consistency in the sense that ``small changes to the tree do not result in large changes to the root''. The notion of ``root may change arbitrarily'' is vague.
\end{reviewer}

\answer Consistency does not ensure that the changes are not big but ensures they are \emph{consistent} by which we mean the root must be on a path between the old root and the newly added node. By saying the root may change arbitrarily, we meant that there might be no relation between roots in a tree and the tree after the change. For instance, one could devise a rooting measure such that for every tree $T$ with an odd number of nodes, assign a root according to closeness centrality, and for trees with an even number of nodes, the root is always a leaf. Such a measure would not be consistent because the jumps (distance-wise) between different roots could be arbitrarily big. We better clarify this in the paper. 

\smallskip

\begin{reviewer}
In section 4: it seems that potential functions measure the potential of a subtree with respect to a specific vertex. Saying that it measures the ``potential of the tree'' is confusing.
\end{reviewer}

\answer Indeed, a potential function assesses a \emph{rooted} tree, i.e., a tree with one node selected and the assessment usually depends on the selection. We prefer to think of potential functions as functions that assess (rooted) trees and not nodes in trees (as centrality measures), as we believe it fits better with the meaning of such functions (height of a tree, number of nodes in a tree, etc.). We clarified this in the text.

\smallskip

\begin{reviewer}
Please explain the equality concerning $|A(u,T)|$ in line 323.
\end{reviewer}

\answer Fix a tree $T$ and two adjacent nodes $u,v$. We want to determine the number of all subgraphs that contain node $u$ in $T$: $|\Asg(u,T)|$. There are $|\Asg(u,T_{u,v})|$ subgraphs that do not contain $v$. Now, if a subgraph contains both $u$ and $v$, then it is a union of a subgraph that contains $u$ in $T_{u,v}$ and a subgraph that contains $v$ in $T_{v,u}$. Hence, there are $|\Asg(u,T_{u,v})| \cdot |\Asg(v,T_{v,u})|$ such subgraphs and we get: $|\Asg(u,T)| = |\Asg(u,T_{u,v})| + |\Asg(u,T_{u,v})| \cdot |\Asg(v,T_{v,u})|$. We decided to maintain the current description in the text as we believe it is good enough to present the main idea. 
\smallskip

\begin{reviewer}
The contribution of Algorithm 1 is not clear. Are there other algorithms that compute the root in less than $O(n^2)$ ? How critical are potential functions for this result ?
\end{reviewer}

\answer For some measures (e.g., degree, closeness) there exist algorithms that are able to find the most central node in time $O(n \log(n))$ or $O(n)$ in trees. For others (e.g., all-subgraphs) our algorithm outperforms existing approaches. The main contribution, however, is a general algorithm that can be applied for any measure defined through a symmetric potential function.

\begin{reviewer}
The paper is quite low on references for a topic so intensively studied, and connections to other works that investigate centrality measures from a theoretical point of  view (perhaps not on trees), seems to be missing.
\end{reviewer}

\answer To the best of our knowledge, the current related work section covers most of the relevant work connected to this paper. Since we removed the motivation on data centrality, the current section covers most of the work related to principles of centrality measures and trees.

%The related work section covers extended the description of other theoretical works on centrality measures and discussed how it relates to our work in ``Related work'' section of the introduction. (TODO - extend and discuss)

\begin{reviewer}
	The framework developed in the paper applies only to trees, which is a very restrictive assumption to make in the context of network analysis. This weakens the motivation of the paper. The authors' claim that this could guide the study of other data models remains unfounded.
\end{reviewer}

\answer We extended the discussion on potential applications of our work. In particular, we discussed how our framework of potential functions can be extended to general graphs in the final section.


\subsection{Response to Reviewer 2}

\begin{reviewer}
	The paper still needs a proofreading pass that cleans up the grammar. The body is in reasonable shape, but introduction and conclusions seem to be written in a hurry.
\end{reviewer}

\answer We thank the reviewer for all his comments and suggestions for improving the grammar, which we followed in this new version. 
%We agree that the introduction and conclusions were not the best in the previous version. % OS I don't think we need to write that
Following reviewers' comment, we have rewritten both sections.

\begin{reviewer}
	The paper is lacking a discussion about the novelty of the complexity to compute centrality measures. It defines a procedure to compute the central node in $O(n \log(n))$ time for a broad class, which is very nice, but is this a new insight for the centrality measures mentioned in the paper? I understand that these are probably studied on graphs, but still. What does the research say? Can they be computed in time $O(n \log(n))$ over graphs? If you run their algorithms from the literature over trees, does this give you $O(n \log(n))$?
\end{reviewer}

\answer For some measures (e.g., degree, closeness, eccentricity) there exist algorithms in the literature that are able to find the most central node in time $O(n \log(n))$ or $O(n)$ in trees. For others (e.g., all-subgraphs) our algorithm outperforms existing approaches. The main contribution, however, is a general algorithm that can be applied for any measure defined through a symmetric potential function.

\begin{reviewer}
l 19-20 The sentence "We show that for all standard centralities..." did not make sense to me at all when I first read the abstract. Maybe it's too deep too soon. Perhaps you want to say that you introduce potential functions in the paper that can be used to characterize certain centrality measures; and that is useful to define an efficient algorithm for a broad class of centrality functions.
\end{reviewer}

\answer We have rewritten the abstract accordingly. 

\begin{reviewer}
l 56 You indeed phrase this sentence kind of question-like, but I'd hammer in the main question more clearly. Especially since you explicitly refer to ``this simple question'' on l 62 and ``similar questions like the one above'' on l 71-72.
\end{reviewer}

\answer Given the new introduction, this sentence was removed.

\begin{reviewer}
l 68-70 It's not clear from the text whether you mean directed or undirected graphs.
\end{reviewer}

\answer We clarify this in the new introduction.


%Detailed comments:
%\begin{itemize}
%	\item l 13 on the data centrality problem $\checkmark$
%	\item l 15 in the case of trees $\checkmark$
%	\item l 19-20 The sentence "We show that for all standard centralities..." did not make sense to me at all when I first read the abstract. Maybe it's too deep too soon. Perhaps you want to say that you introduce potential functions in the paper that can be used to characterize certain centrality measures; and that is useful to define an efficient algorithm for a broad class of centrality functions.
%	\item l 56 You indeed phrase this sentence kind of question-like, but I'd hammer in the main question more clearly. Especially since you explicitly refer to "this simple question" on l 62 and "similar questions like the one above" on l 71-72.
%	\item l 64 is fundamental to any theory $\checkmark$
%	\item l 68-70 It's not clear from the text whether you mean directed or undirected graphs.
%	\item l 76 which centrality measures always select   (this is a bit clearer) $\checkmark$
%	\item l 77 do you mean tree instead of graph? $\checkmark$
%	\item l 79 which states that $\checkmark$
%	\item l 84 say that such $\checkmark$
%	\item l 90 show that most $\checkmark$
%	\item l 147 such an approach $\checkmark$
%	\item l 170 fix an enumerable $\checkmark$
%	\item l 178 a \emph{path} $\checkmark$
%	\item l 184 between every pair   
%	(Generally, avoid the use of "any". In natural language, its meaning is sometimes a universal and sometimes an existential quantifier, so this is confusing in formal texts.) $\checkmark$
%	\item l 200 vertex that minimizes $\checkmark$
%	\item l 201 You mean $d_G(v,u)$ here, right? (Also, the distance here is always infinite if G is not connected. Is that what you mean? Or do you want to discuss the case for connected G here?)$\checkmark$
%	\item l 202 The sentence "Then, the radius ..." doesn't seem to belong here. $\checkmark$
%	\item l 203 Now, centrality measure [10] selects the center $\checkmark$
%	\item l 204 subgraphs of G that contain v $\checkmark$
%	\item l 213 and all previous $\checkmark$
%	\item l 233 any -> every $\checkmark$
%	\item l 233 \ldots $\checkmark$
%	\item l 241 with an even $\checkmark$
%	\item l 248 on the other hand ? $\checkmark$
%	\item l 249 roots trees $\checkmark$
%	\item l 264 intuition in (no comma) $\checkmark$
%	\item l 277 implies that isomorphic $\checkmark$
%	\item l 281 vertices i and n-1-i $\checkmark$
%	\item l 282 to all symmetric  $\checkmark$  (Here "any" is even grammatically incorrect.)
%	\item l 298 What do closeness [...] have in common?   (Delete "that they root trees" - it's confusing.) $\checkmark$
%	\item l 302 Closure of f under isomorphism is not defined
%	\item l 302 and all adjacent vertices
%	\item l 310 that $f_d$ (no comma) $\checkmark$
%	\item l 311 it also has $\checkmark$
%	\item l 316 which results $\checkmark$
%	\item l 325 the potential function $\checkmark$
%	\item l 330 The table at $\checkmark$
%	\item l 335 Can you explain why this is a natural question?
%	\item l 347 the at-most-one-parent property $\checkmark$
%	\item l 348,354 different spellings of "neighbor" $\checkmark$
%	\item l 358 always has less $\checkmark$
%	\item l 359 Here you have a font issue. The x's in different font should refer to the same object. $\checkmark$
%	\item l 366 that root trees $\checkmark$
%	\item l 367 exists a measure that roots trees $\checkmark$
%	\item l 377 You can be more informative here. What about "under some assumptions on the efficiency to compute the potential function" $\checkmark$
%	\item l 416 moves towards $\checkmark$
%	\item l 437 over all vertices $\checkmark$
%	\item l 448 arbitrarily $\checkmark$
%	\item l 469 consistently roots trees $\checkmark$
%	\item l 536 satisfy properties $\checkmark$
%	\item l 570 by the so-called potential
%	\item l 570 roots trees, i.e., each tree has at most $\checkmark$
%	\item l 571 vertices, referred to as the "roots" $\checkmark$
%	\item l 574 "with good properties" is very vague
%	\item l 577 how do centralities $\checkmark$
%\end{itemize}


\subsection{Response to Reviewer 3}

\begin{reviewer}
	No doubt that data centrality has relevance to databases and while the authors explain this connection and present examples, I do not see the broad picture - where is this work positioned in the broad and well established work on centrality measures? Though the authors do try to compare their work with other works on centrality, I do not fully understand what is the novelty and importance of this work. For instance, the authors say ``this research line does not consider the foundational aspects of these rankings'' - what are the foundational aspects considered in this work that are not considered in previous ones? Another point mentioned by the authors in this context: ``we propose several properties specific for trees and study which are satisfied by standard centrality measures'' - see (3)
\end{reviewer}

\answer Indeed, in recent years theoretical study on centrality measures became an active line of research. The main novelty of our work is focusing on trees: as far as we know, our work is the first theoretical study on centrality measure for trees. 
One of the benefit of our approach is the fact that on trees we were able to identify similarities between centralities from different classes which act very differently on general graphs.
In particular, betweenness, closeness and all-subgraphs centralities all comes from different classes of centralities (medial, distance-based and vitality centrality measures), but as we show they all have potential functions.
We discussed it in the new version of introduction.

\begin{reviewer}
	The paper aims to serve as the basis of future research on centrality measures in DBs, therefore I would expect to see a better justification on why this work is specific to databases (e.g., what aspects of databases are taken into account here that are not taken into account in other works on data centrality).
\end{reviewer}

\answer We agree that the previous motivation on data centrality was not correctly justified. For this reason, we change the motivation of the abstract and introduction. In the introduction, we present more uses of centrality measures in data management systems regarding the connection to databases. Furthermore, we added a section at the end of the paper showing possible applications of potential functions in databases. It is important to mention that the contribution of our work is on the principles of data management systems, and, then, it was not our purpose to aim this work on applications. Nevertheless, we agree that showing possible applications in the paper helps the reader better understand how these results are connected with database systems.

\begin{reviewer}
	The focus on trees seems problematic to me. Though the authors do acknowledge this and say ``the most relevant problems regarding data centrality are for graph data or relational data'', they choose to focus only on trees. I do not find the authors’ justification very convincing since if one wants to talk about data centrality in the context of DBs it is only natural to focus on models that are really used by DBMSs. It is indeed a good strategy to study simpler models before more complex ones but this weakens the connection and relevance to DBs. This also makes me wonder whether the paper is not more compatible with an algorithmic conference rather than a DB conference.
\end{reviewer}

\answer The focus on trees has two main advantages. In first place, the axiomatic approach for centrality measures is always a study over general graphs but for a very few types of centrality measures. Our work, on the opposite, focused on a very restricted (and simpler) set of graphs but we were able to compare very different (in spirit) measures under the same scope (rooting trees). In second place, as the reviewer said, the simpler structure of trees allowed us to have a deeper and fundamental understanding of centrality. Therefore, even if we refer to a an uncommon data structure, understanding data centrality over trees is a necessary step in order to generalize it. Some applications of data centrality for trees are discussed in the final section.

\begin{reviewer}
	The main ideas presented in the paper on potential functions and consistency are only applicable to trees. So I do not see how this work can be extended to more interesting models such as graphs or relational data.
\end{reviewer}

\answer We discussed how our framework of potential functions can be extended to general graphs in the final section.

